On Hybrid Radar Fusion for Integrated Sensing and Communication

The following paper introduces a novel integrated sensing and communication (ISAC) scenario termed hybrid radar fusion. In this setting, the dual-functional radar and communications (DFRC) base station (BS) acts as a mono-static radar in the downlink (DL), for sensing purposes, while performing its DL communication tasks. Meanwhile, the communication users act as distributed bi-static radar nodes in the uplink (UL) following a frequency-division duplex protocol. The DFRC BS fuses the information available at different DL and UL resource bands to estimate the angles-of-arrival (AoAs) of the multiple targets existing in the scene. In this work, we derive the maximum likelihood (ML) criterion for the hybrid radar fusion problem at hand. Additionally, we design efficient estimators; the first algorithm is based on an alternating optimization approach to solve the ML criterion, while the second one designs an optimization framework that leads to an alternating subspace approach to estimate AoAs for both the target and users. Finally, we demonstrate the superior performance of both algorithms in different scenarios, and the gains offered by these proposed methods through numerical simulations.

==> Response2/C1o1.tex <==
The authors would like to thank the reviewer for the comment.
We have conducted a simulation by utilizing typical values of a \ac{mmWave} communication system \cite{8207426}.
%% what are the general cases where we are right and the fusion is good. 
We observe that at a transmit power of $40\dBm$, equivalent to the transmit power of a base station in typical millimeter-wave systems \cite{8207426}, the \ac{HRF} consistently provides substantial sensing benefits as the number of users increases. 
To illustrate, with no users ($K = 0$), the \ac{CRB} stands at $0.13 \rad^2$, and as we introduce a single user ($K = 1$), the \ac{CRB} decreases to $0.1\rad^2$. 
Scaling up to $4$ users, a proportional reduction factor of $2$ is maintained, resulting in CRB values of $0.05 \rad^2$, followed by a \ac{CRB} of $0.025\rad^2$ for $K = 16$ users.
%% And then say, is SOME CASES, and you explain what are these cases, the fusion may not be needed.
In some other cases, where the user transmits at significantly lower power and utilizes a smaller antenna array compared to the \ac{DFRC} \ac{BS}, it's observed that the BS-target-BS link can exhibit considerably larger receive power than the user-target-BS link.
In such as case, the fusion may not be needed.
%The necessity to fuse the received signals from these links can be influenced by the disparities in power and antenna configurations, as discussed in the analysis below.
The simulation performed demonstrates the critical relationship between transmit power levels and the performance enhancements brought by the \ac{HRF} scheme. 
It suggests that in scenarios where the transmit power surpasses certain thresholds, the utilization of HRF might not yield substantial additional sensing gains beyond the capabilities of the base station operating independently.
In particular, we observe that at $52\dBm$ of transmit \ac{DFRC} power, the \ac{HRF} \ac{CRB} for $K = 1$ coincides with the \ac{DFRC} \ac{BS} operating along (i.e. no fusion occurs). 
Likewise, when the \ac{DFRC} \ac{BS} utilizes at least $66\dBm$ transmit  power, then it is not necessary to fuse the received signals for $K = 4$.
In addition, when transmit power exceeds $78\dBm$, then it is not necessary to fuse the received signals for $K = 16$ users.
%% 


==> Response2/C1o2.tex <==
The authors would like to thank the reviewer for the comment.
The signal after reflection will indeed have much less power in general due to the double path-loss, and this will limit the detection performance, if not pragmatically dealt with.
%    - ADC optimization, maybe, but i wanna get a better feel to see that if we optimize few-bit ADCs, can we see very weak paths ? I think we can see weak paths but not very weak 
A promising direction that we are currently working on is the integration of an \ac{ADC} model ($1$-bit or few-bit) by mapping the analog signal in equation \eqref{eq:rx-OFDM-UL} to equation \eqref{eq:sample-rx-OFDM} of the manuscript via the \ac{ADC} function $\mathcal{Q}(.)$ (e.g. uniform mid-rise quantizer \cite{8171203} or the extreme 1-bit \ac{ADC} case, i.e. a simple comparator \cite{mezghani2018blind}) that would allow us to analyze the estimation limits as a function of ratios of user-BS to user-target-BS powers, in practical systems.
We are motivated by the interesting proof-of-concept work in \cite{9054740}, where it has been shown that a \ac{GAMP} algorithm with $1$-bit \ac{ADC} can see reflections with a dynamic range of $35\dB$ instead of $50\dB$ with $12$-bit \ac{ADC} used in the testbed in \cite{9135453}.
We can learn that sophisticated estimation algorithms tailored for $1$-bit, or even few-bit \acp{ADC}, can help us make use of weak paths in our \ac{HRF} context, especially when different users are contributing to more paths on their allocated frequency bands. 
%so user-BS (ignoring the bounces) we know how to answer, power control like the 2-3 papers you shared
In addition, to address the links between different users and BS, we also highlight that a user should not overwhelm other weaker users and this can be realized through some power control mechanism \cite{7931630}, which is of good advantage for low-resolution \ac{ADC} structures \cite{7894211}.
%we must assume that some type of power control is implemented that prevents a strong user from overwhelming other weaker users.
%- user-BS vs. bounce, many options: 
%    - do like PR as we said ( add references and say this is a common problem in PR ) 
Besides developing algorithms, we aim to illuminate the interconnection of this issue with a classical bi-static problem in the radar community, namely the \ac{DPI} problem \cite{malanowski2019signal} (c.f. Section 2.3.3). 
The problem of \ac{DPI} is that the direct \ac{LoS} between the transmitting and receiving units of the bistatic system is stronger relative to the very weak target echoes. 
A typical solution that has been commonly proposed in the literature is analog suppression, e.g. through effective receiver radiation pattern and analog \ac{DPIS} cancellation \cite{peto2018analog}.



==> Response2/C1o3.tex <==
We would like to thank the reviewer for the comment.
We have conducted another simulation regarding this to see when does it seem reasonable to abandon the smaller paths and just focus on the larger ones. 
In the general case, our simulations show that for reasonable ratio of reflection power to LoS power, the \ac{HRF} gains are still pronounced especially when increasing number of communication users.
In the extreme case, where the reflection power is very small then we can abandon those links.
In particular, our findings reveal that for a typical \ac{mmWave} communication system \cite{8207426} when on average the reflection power is $90\dB$ less than the \ac{LoS} power, then one should abandon the reflections and focus on the \ac{LoS} when $K = 1$ user is present. 
When $K = 4$ communication users are there, then the average reflection to \ac{LoS} power beyond $-96\dB$ does not bring useful information to \ac{HRF}. 
Likewise, when reflection-to-LoS ratio is less than $-102\dB$, then one may abandon the smaller ones as it does not bring additional gain when compared to the \ac{DFRC} \ac{BS} in standalone. 




%"When the reflection-to-LoS ratio is less than $-90\dB$, we see that $K = 1$ users coincides with that of the \ac{DFRC} \ac{BS} only-case.
%When the reflection-to-LoS ratio is less than $-96\dB$, we see that $K = 4$ users coincides with that of the \ac{DFRC} \ac{BS} only-case.
%When the reflection-to-LoS ratio is less than $-102\dB$, we see that $K = 16$ users coincides with that of the \ac{DFRC} \ac{BS} only-case."

==> Response2/C2_minor.tex <==
Thank you for pointing this out.
We have taken the necessary action to highlight this RCS change.

==> Response2/C3_minor.tex <==
% It seems that (31) and (32) are not equivalent.
We start by expanding \eqref{eq:maximum-likelihood-4} as follows
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmin_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{p,k}
	\big\Vert 
	\pmb{Y}_k(:,p) 
	-
	\pmb{P}_k
	\pmb{Y}_k(:,p)
	\big\Vert^2,
\end{equation}	
\begin{equation}
\begin{split}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
&=
	\argmin_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{p,k}
	\Big[
\Vert 
	\pmb{Y}_k(:,p)
\Vert^2
	-
	( \pmb{Y}_k(:,p) )^H
	\pmb{P}_k
	\pmb{Y}_k(:,p)
	-
(	\pmb{P}_k
	\pmb{Y}_k(:,p)
	)^H
	\pmb{Y}_k(:,p) 
	+
\Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2
	\Big]
\end{split}
\end{equation}
Due to the fact that $\pmb{P}_k^H = \pmb{P}_k$, the above equation can be written as 
\begin{equation}
\label{eq:step3}
\begin{split}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
&=
	\argmin_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{p,k}
	\Big[
\Vert 
	\pmb{Y}_k(:,p)
\Vert^2
	-
	2
	( \pmb{Y}_k(:,p) )^H
	\pmb{P}_k
	\pmb{Y}_k(:,p)
+
\Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2
	\Big]
\end{split}
\end{equation}
Utilizing the idempotent property of $\pmb{P}_k$, namely $\pmb{P}_k=\pmb{P}_k\pmb{P}_k$, we can say that
\begin{equation}
\label{eq:idempotent}
	( \pmb{Y}_k(:,p) )^H
	\pmb{P}_k
	\pmb{Y}_k(:,p) = \Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2
\end{equation}
Therefore using \eqref{eq:idempotent} in \eqref{eq:step3}, we obtain
\begin{equation}
\begin{split}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
&=
	\argmin_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{p,k}
	\Big[
\Vert 
	\pmb{Y}_k(:,p)
\Vert^2
-
\Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2
	\Big]
\end{split}
\end{equation}
Since $\pmb{Y}_k(:,p)$ is independent of the variables we are optimizing for, i.e. they are the observation samples, therefore, we can say
\begin{equation}
\begin{split}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
&=
	\argmin_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
-
	\sum\nolimits_{p,k}
\Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2
\end{split}
\end{equation}
Since $\Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2$ is a non-negative quantity, then minimizing $- \Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2$ is the equivalent of maximizing $\Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2$, hence we have 
\begin{equation}
\begin{split}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
&=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{p,k}
\Vert 
		\pmb{P}_k
	\pmb{Y}_k(:,p)
\Vert^2
\end{split}
\end{equation}
which is equation \eqref{eq:maximum-likelihood-5} in the updated manuscript (previously equation (32)).


%In addition, how to obtain (33) based on (32) is not clear. 
Now let us expand  equation \eqref{eq:maximum-likelihood-5} in the updated manuscript (previously equation (32)), we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{k}
	\sum\nolimits_{p}
(	\pmb{P}_k
	\pmb{Y}_k(:,p))^H
	\pmb{P}_k
	\pmb{Y}_k(:,p)
\end{equation} 
which can be written as 
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{k}
	\sum\nolimits_{p}
	\pmb{Y}_k(:,p)^H
	\pmb{P}_k^H
	\pmb{P}_k
	\pmb{Y}_k(:,p)
\end{equation} 
Using $\pmb{P}_k^H = \pmb{P}_k$ and $\pmb{P}_k=\pmb{P}_k\pmb{P}_k$, we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{k}
	\sum\nolimits_{p}
	\pmb{Y}_k(:,p)^H
	\pmb{P}_k
	\pmb{Y}_k(:,p)
\end{equation} 
Since $	\pmb{Y}_k(:,p)^H
	\pmb{P}_k
	\pmb{Y}_k(:,p)$ is a scalar, we can introduce the trace operator directly as
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{k}
	\sum\nolimits_{p}
	\trace 
	\Big(
	\pmb{Y}_k(:,p)^H
	\pmb{P}_k
	\pmb{Y}_k(:,p)
	\Big)
\end{equation} 
Using $\trace(\pmb{A}\pmb{B}) = \trace(\pmb{B}\pmb{A})$, we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{k}
	\sum\nolimits_{p}
	\trace 
	\Big(
	\pmb{P}_k
	\pmb{Y}_k(:,p)
	\pmb{Y}_k(:,p)^H
	\Big)
\end{equation}
Using $\trace(\pmb{A}+\pmb{B}) = \trace(\pmb{A}) + \trace(\pmb{B})$, we can absorb the summation over $p$ within the trace operator as 
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{k}
	\trace 
	\Big(
	\pmb{P}_k
	\sum\nolimits_{p}
	\pmb{Y}_k(:,p)
	\pmb{Y}_k(:,p)^H
	\Big)
\end{equation}
Using $	\sum\nolimits_{p}
	\pmb{Y}_k(:,p)
	\pmb{Y}_k(:,p)^H = 	\pmb{Y}_k
	\pmb{Y}_k^H$, we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{k}
	\trace 
	\Big(
	\pmb{P}_k
	\pmb{Y}_k
	\pmb{Y}_k^H
	\Big)
\end{equation}	
By using equation \eqref{eq:sample-covariance-matrix} in the updated manuscript, we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\sum\nolimits_{k}
	\trace 
	\Big(
	\pmb{P}_k
	\widehat{\pmb{R}}_k
	\Big)
\end{equation}	
which is equation \eqref{eq:maximum-likelihood-6} in the updated manuscript (previously equation (33)).

% Moreover, how to obtain (37) based on (33) is also not clear.

Splitting the summation in equation \eqref{eq:maximum-likelihood-6} in the updated manuscript (previously equation (33)), we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\Big[
	\trace 
	\Big(
	\pmb{P}_0
	\widehat{\pmb{R}}_0
	\Big)
	+
	\sum\nolimits_{k=1}^K
	\trace 
	\Big(
	\pmb{P}_k
	\widehat{\pmb{R}}_k
	\Big)
	\Big],
\end{equation}	
Plugging equation \eqref{eq:projec-matr-decomp} of the updated manuscript in the above, we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\Big[
	\trace 
	\Big(
	\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_0)}
	\widehat{\pmb{R}}_0
	\Big)
	+
	\sum\nolimits_{k=1}^K
	\trace 
	\Big(
	(\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)} 
		+
		\pmb{P}_{
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})})
	\widehat{\pmb{R}}_k
	\Big)
	\Big],
\end{equation}	
Expanding the second term and using $\trace[(\pmb{A} + \pmb{B})\pmb{C}] = \trace(\pmb{A}\pmb{C}) + \trace(\pmb{B}\pmb{C})$, we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\Big[
	\trace 
	\Big(
	\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_0)}
	\widehat{\pmb{R}}_0
	\Big)
	+
	\sum\nolimits_{k=1}^K
	\trace 
	\Big(
	\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)} 
	\widehat{\pmb{R}}_k
	\Big)
		+
		\sum\nolimits_{k=1}^K
		\trace 
	\Big(
		\pmb{P}_{
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})}
	\widehat{\pmb{R}}_k
	\Big)
	\Big],
\end{equation}	
The first two terms can be written using one sum, hence,
\begin{equation}
\label{eq:equation37-in-mid-way}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\Big[
	\sum\nolimits_{k=0}^K
	\trace 
	\Big(
	\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)} 
	\widehat{\pmb{R}}_k
	\Big)
		+
		\sum\nolimits_{k=1}^K
		\trace 
	\Big(
		\pmb{P}_{
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})}
	\widehat{\pmb{R}}_k
	\Big)
	\Big],
\end{equation}	
Expanding the projector $\pmb{P}_{
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})}$ by using $\pmb{P}_{\pmb{A}} = \pmb{A}(\pmb{A}^H \pmb{A})^{-1} \pmb{A}^H$ as follows
\begin{equation}
\label{eq:null-projector-overAu}
	\pmb{P}_{
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})}
		=
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})
		\Bigg(
\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} 
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} 
\pmb{a}(\theta_k^{\tt{u}})
		\Bigg)^{-1}
\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp}
\end{equation}
where, in the above equation, we have used $(\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp})^H = \pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp}$.
Moreover, since $\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} $ is itself a projector therefore it is idempotent, hence $\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} 
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp}  = \pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} $. Therefore, equation \eqref{eq:null-projector-overAu} herein can be written as 
\begin{equation}
\label{eq:null-projector-overAu-2}
	\pmb{P}_{
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})}
		=
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})
		\Bigg(
\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} 
\pmb{a}(\theta_k^{\tt{u}})
		\Bigg)^{-1}
\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp}
\end{equation}
Since the quantity appearing within the inverse is a scalar, we get
\begin{equation}
\label{eq:null-projector-overAu-3}
	\pmb{P}_{
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})}
		=
		\frac{1}{\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} 
\pmb{a}(\theta_k^{\tt{u}})}
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})
\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp}
\end{equation}
Plugging equation \eqref{eq:null-projector-overAu-3} herein into equation \eqref{eq:equation37-in-mid-way} herein, we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\Big[
	\sum\nolimits_{k=0}^K
	\trace 
	\Big(
	\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)} 
	\widehat{\pmb{R}}_k
	\Big)
		+
		\sum\nolimits_{k=1}^K
		\frac
{		\trace 
	\Big(
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} \pmb{a}(\theta_k^{\tt{u}})
\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp}
	\widehat{\pmb{R}}_k
	\Big)}
{\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} 
\pmb{a}(\theta_k^{\tt{u}})}
	\Big],
\end{equation}	
Using the circular property of the trace, namely $\trace(\pmb{A}\pmb{B}) = \trace(\pmb{B}\pmb{A})$, twice we get
\begin{equation}
\big\lbrace 
\widehat{\pmb{\Theta}}^{\tt{tar}},
\widehat{\pmb{\Theta}}^{\tt{u}} 
\big\rbrace
=
	\argmax_{\lbrace \pmb{\Theta}^{\tt{tar}} , \pmb{\Theta}^{\tt{u}} \rbrace }
	\Big[
	\sum\nolimits_{k=0}^K
	\trace 
	\Big(
	\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)} 
	\widehat{\pmb{R}}_k
	\Big)
		+
		\sum\nolimits_{k=1}^K
		\frac
{		\trace 
	\Big(
\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp}
	\widehat{\pmb{R}}_k
		\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} 
		\pmb{a}(\theta_k^{\tt{u}})
	\Big)}
{\pmb{a}^H(\theta_k^{\tt{u}})
\pmb{P}_{\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)}^{\perp} 
\pmb{a}(\theta_k^{\tt{u}})}
	\Big],
\end{equation}
Since the argument within the trace is a scalar, then we can remove the trace operator, hence we get equation \eqref{eq:maximum-likelihood-7} in the updated manuscript (previously equation (37)).
Due to the very limited space, we have omitted the details.










==> Response2/C6_minor.tex <==
The authors would like to thank the reviewer for the comment.
Indeed, the content was missing.


First, we obtain $\widehat{\pmb{U}}_{N,0}$ by computing the sample covariance matrix $\widehat{\pmb{R}}_0$ following equation \eqref{eq:sample-covariance-matrix} of the updated manuscript (for $k = 0$), then by performing \ac{EVD} as shown in equation \eqref{eq:EVD-on-sample-covariance-matrix} of the updated manuscript (for $k = 0$). In particular, referring to equation \eqref{eq:EVD-on-sample-covariance-matrix}, we can extract $\widehat{\pmb{U}}_{N,0} \in \mathbb{C}^{N \times (N - \vert \Phi_0 \vert)}$. Now that we have $\widehat{\pmb{U}}_{N,0}$, we compute $\widehat{\pmb{P}}_0^{\perp}	$ in equation \eqref{eq:initial-null-space} of the updated manuscript (previously equation (49)).

Second, to obtain $\widehat{\bar{\pmb{R}}}_k$ in equation \eqref{eq:estimated-projected-covariance-phase-one} of the updated manuscript (previously equation (50)), we utilize $\widehat{\pmb{P}}_0^{\perp}$ of equation \eqref{eq:initial-null-space} in order to multiply $\widehat{\pmb{R}}_k$, is obtained equation \eqref{eq:sample-covariance-matrix} of the updated manuscript for all $k$.

The following text has been added below equation \eqref{eq:estimated-projected-covariance-phase-one} of the updated manuscript:\\

\textcolor{blue}{\input{actions02/obtaining-49-50.tex}}





==> Response2/C7_minor.tex <==
Thank you for pointing out the typo.
The sentence "It is also assumed that the downlink consists of $L_0$ OFDM symbols." has been replaced by 
\textcolor{blue}{\input{actions02/consists-of-l0-ofdm-replacement.tex}}
Other typos have also been corrected in the manuscript.

==> actions01/HAD/had.tex <==
%\documentclass{article}
%% \documentclass[12pt, draftclsnofoot, onecolumn]{IEEEtran}
%\usepackage{amsmath,amsfonts}
%%\usepackage{algpseudocode}
%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{array}
%\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\usepackage{textcomp}
%\usepackage{stfloats}
%\usepackage{url}
%\usepackage{verbatim}
%\usepackage{color,soul}
%\usepackage{graphicx}
%\usepackage{hyperref}
%\usepackage{cite}
%\usepackage[nolist]{acronym}
%\usepackage{mathtools}
%\usepackage{amssymb}
%\acrodefplural{HPA}[HPAs]{high power amplifiers}
%
%
%
%\DeclareMathOperator{\Span}{span}
%\DeclareMathOperator{\trace}{tr}
%\DeclareMathOperator{\SNR}{SNR}
%\DeclareMathOperator{\SINR}{SINR}
%\DeclareMathOperator{\MUI}{MUI}
%\DeclareMathOperator{\PAPR}{PAPR}
%\DeclareMathOperator{\comm}{comm}
%\DeclareMathOperator{\ve}{vec}
%\DeclareMathOperator{\Real}{Re}
%\DeclareMathOperator{\Imag}{Im}
%\DeclareMathOperator{\dB}{dB}
%\DeclareMathOperator{\opt}{opt}
%\DeclareMathOperator{\svd}{SVD}
%\DeclareMathOperator{\MSE}{MSE}
%\DeclareMathOperator{\rad}{rad}
%\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\CRB}{CRB}
%
%%\DeclareMathOperator{\span}{span}
%
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%
%\newcommand\myeqa{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily (a)}}}{=}}}
%\newcommand\myeqb{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily (b)}}}{=}}}
%\newcommand\myeqc{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily (c)}}}{=}}}
%\newcommand\myeqd{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily (d)}}}{=}}}
%
%
%\newcommand\myleqa{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily (a)}}}{\leq}}}
%\newcommand\myleqb{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily (b)}}}{\leq}}}
%\newcommand\myleqc{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily (c)}}}{\leq}}}
%\newcommand\myleqd{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily (d)}}}{\leq}}}
%
%
%\makeatother
%
%
%
%
%\begin{document}
\begin{figure}[!t]
\centering
\includegraphics[width=4.5in]{./actions01/HAD/HAD-figure.pdf}
\caption{\textcolor{darkgreen}{A Hybrid Analog Beamformer well-suited for the hybrid radar fusion design.}}
\label{fig:HAD-BFer}
\end{figure}
Consider a hybrid beamformer divided into sub-arrays, each of size $P$, with a total number of $N$ RF chains. Therefore a total of $NP$ antennas are placed. Let's denote by $w_p^{(n)}$ the $p^{th}$ phase shifting element within the $n^{th}$ sub-array. The goal of this hybrid beamformer would be to adjust the gains the of target reflections to match the LoS coming from the users. 
Note that this can be seen as spatial oversampling by a factor of $P$. 	

Denoting the phase shifts at the $n^{th}$ sub-array as 
\begin{equation}
	\pmb{w}^{(n)}
	=
	\begin{bmatrix}
		w_1^{(n)} & \ldots & w_P^{(n)}
	\end{bmatrix}^T,
\end{equation}
we can propose the following analog beamformer 

\begin{equation}
 \label{eq:problem3}
\begin{aligned}
(\mathcal{A}):
\begin{cases}
\min\limits_{ \lbrace w_p^{(n)} \rbrace_{n,p} , \alpha \in \mathbb{C} }& 	\sum\limits_{n=1}^N
	\sum\limits_{\theta \in \mathcal{G}}
	\Vert 
	y(\theta) 
	a_n(\theta) 
	-
	\alpha \pmb{b}_n^H(\theta)
	\pmb{w}^{(n)}
	\Vert^2   \\
\textrm{s.t.}
 & \vert w_p^{(n)} \vert = 1, p = 1\ldots P, \quad n = 1\ldots N,
\end{cases}
\end{aligned}
\end{equation}
where $\alpha$ is scaling complex variable that can be used in the amplification process with  and $\pmb{b}_n(\theta)$ is the array response of the $n^{th}$ sub-array, and hence the total array response is 
\begin{equation}
	\pmb{b}(\theta)
	=
	\begin{bmatrix}
		\pmb{b}_1(\theta) & \ldots & \pmb{b}_N(\theta)
	\end{bmatrix}^T,
\end{equation}
The hybrid beamforming problem in \eqref{eq:problem3} aims at fitting the output of each subarray to the steering vector in direction $y(\theta)\pmb{a}_n(\theta)$. The amplitudes $y(\theta)$ being direction-dependent are key to adjusting power levels between the sector defined for radar operations, i.e. $\pmb{\Omega}_r$, versus all other directions (namely LoS communications). Radar operation in this case means that we are interested in exploring targets that only lie within $\pmb{\Omega}_r$. Assuming that, due to double path-loss, the gap between LoS power and the reflection power is $\kappa_{\tt{high}}-\kappa_{\tt{low}}$, then we would have to compensate that loss within the radar sector, i.e. we choose
\begin{equation}
\label{eq:y-theta}
	y(\theta)
	=
	\begin{cases}
		\kappa_{\tt{high}} , & \text{if } \theta \in \pmb{\Omega}_r \\
		\kappa_{\tt{low}}, & \text{else}
	\end{cases}.
\end{equation}
With this modeling, we desire that if a single impinges the antenna array at $\pmb{b}(\theta)$, then the output of the $N$ sub-arrays would be $\kappa_{\tt{high}} \pmb{a}(\theta) \in \mathbb{C}^{N \times 1}$, if $\theta \in \pmb{\Omega}_r$, otherwise it would be $\kappa_{\tt{low}} \pmb{a}(\theta)$.

In Fig. \ref{fig:HAD-BFer}, we show the design of the hybrid analog beamformer, where the hybrid radar fusion can specify a desired radar operation sector $ \pmb{\Omega}_r$, which then sets the $y(\theta)$ according to \eqref{eq:y-theta} for a given $\kappa_{\tt{low}},\kappa_{\tt{high}}$, which runs the majorization-minimization (MM) solver to set the weights of the hybrid analog beamformer. 


Having this mind, then we aim at finding the best phase shifts and the scale $\alpha$, so that $y(\theta)\pmb{a}(\theta)$ matches 
$\alpha \begin{bmatrix}
	\pmb{b}_1^H(\theta)
	\pmb{w}^{(1)} & 
	\ldots
	&
	\pmb{b}_N^H(\theta)
	\pmb{w}^{(N)}
\end{bmatrix}^T$. Therefore, for evaluation, we also feel that the spatial term $g(\theta)$ defined below
\begin{equation}
	\label{eq:spatial-term}
	g(\theta)
	=
	\Vert
	y(\theta)\pmb{a}(\theta)
	-
	\alpha_{\tt{opt}} \begin{bmatrix}
	\pmb{b}_1^H(\theta)
	\pmb{w}_{\tt{opt}}^{(1)} & 
	\ldots
	&
	\pmb{b}_N^H(\theta)
	\pmb{w}_{\tt{opt}}^{(N)}
\end{bmatrix}^T
\Vert^2
\end{equation}
allows us to assess the suitability of the phase shifters for the hybrid radar fusion estimation process. In the above, $\alpha_{\tt{opt}}$ and $\pmb{w}_{\tt{opt}}^{(1)} \ldots \pmb{w}_{\tt{opt}}^{(N)}$ are the optimal solutions given by our iterative solver described in equations \eqref{eq:MM-iter-1} and \eqref{eq:MM-iter-2}.

Furthermore, an important note here is that we consider only a one-dimensional spatial aspect ($\theta$ being only an azimuth spatial view) for sake of simplicity and compact representation. That said, we can extend to 2D to allow a 3D view of the environment through both azimuth and elevation (in that case, the manuscript as well as the methods in the response letter can be easily extended by replacing $\theta$, with $\theta,\phi$ (where $\phi$ is elevation) and using $2D$ planar arrays, like uniform planar arrays).
To this end, we can re-express \eqref{eq:problem3} in a more compact way as 
\begin{equation}
 \label{eq:problem4}
\begin{aligned}
(\mathcal{A}):
\begin{cases}
\min\limits_{\lbrace w_p^{(n)} \rbrace_{n,p}, \alpha \in \mathbb{C} }& 	
\sum\limits_{n=1}^N	
	\Vert 
	\pmb{y}_n 
	-
	\alpha
	\pmb{B}_n
	\pmb{w}^{(n)}
	\Vert^2   \\
\textrm{s.t.}
 & \vert w_p^{(n)} \vert = 1, p = 1\ldots P, \quad n = 1\ldots N,
\end{cases}
\end{aligned}
\end{equation}
where 
\begin{equation}
	\pmb{y}_n = \begin{bmatrix}
	y(\theta_1) 
	a_n(\theta_1) &
	y(\theta_2) 
	a_n(\theta_2) & 
	\ldots
	&
y(\theta_{\vert \mathcal{G} \vert}) 
	a_n(\theta_{\vert \mathcal{G} \vert})
\end{bmatrix}^T
\end{equation} and 
\begin{equation}
	\pmb{B}_n
=
\begin{bmatrix}
	\pmb{b}_n(\theta_1)
	&
	\pmb{b}_n(\theta_2)
	 & 
	\ldots
	&
\pmb{b}_n(\theta_{\vert \mathcal{G} \vert})
\end{bmatrix}^H
\end{equation}
Finally, we write problem \eqref{eq:problem4} in its most compact version as 
\begin{equation}
 \label{eq:problem5}
\begin{aligned}
(\mathcal{A}):
\begin{cases}
\min\limits_{\pmb{w},\alpha \in \mathbb{C}}& 	
	\Vert 
	\pmb{y}
	-
	\alpha
	\pmb{B}
	\pmb{w}
	\Vert^2   \\
\textrm{s.t.}
 & \vert w_p^{(n)} \vert = 1, p = 1\ldots P, \quad n = 1\ldots N,
\end{cases}
\end{aligned}
\end{equation}
where $\pmb{y} = 
\begin{bmatrix}
	\pmb{y}_1^T & \pmb{y}_2^T & \ldots & \pmb{y}_N^T
\end{bmatrix}^T$, $\pmb{w} = 
\begin{bmatrix}
	(\pmb{w}^{(1)})^T & (\pmb{w}^{(2)})^T & \ldots & (\pmb{w}^{(N)})^T
\end{bmatrix}^T$, and 
\begin{equation}
	\pmb{B} = \blkdiag(\pmb{B}_1 , \pmb{B}_2 \ldots \pmb{B}_N)
\end{equation}
where $\blkdiag$ is the block-diagonal operator. Now, the problem in \eqref{eq:problem5} is non-convex with respect to the phase shifts $\pmb{w}$ due to the phase shift constraint (i.e. $\vert w_p^{(n)} \vert = 1$). For that, we can solve \eqref{eq:problem5} through a majorization-minimization (MM) approach. To this end, denote the function 
\begin{equation}
	f(\alpha, \pmb{w})
	=
	\Vert 
	\pmb{y}
	-
	\alpha
	\pmb{B}
	\pmb{w}
	\Vert^2
\end{equation}
The MM technique decomposes the problem into two subproblems, i.e.
\begin{equation}
	\label{eq:MM-1}
	\alpha^{[m+1]}
	=
	\argmin_{\alpha \in \mathbb{C}}
	f(\alpha, \pmb{w}^{[m]})
\end{equation}
and
\begin{equation}
	\label{eq:MM-2}
	\pmb{w}^{[m+1]}
	=
	\argmin_{\pmb{w} \in \mathcal{P}^{NP}}
	f(\alpha^{[m+1]}, \pmb{w})
\end{equation}
where $ \mathcal{P}^{NP}$ is the space containing all vectors $\pmb{x} \in \mathbb{C}^{NP \times 1}$ such that their magnitude is $1$ (which is basically the feasible set of problem \eqref{eq:problem5}). First, solving \eqref{eq:MM-1}, the problem can be easily solved as $f$ is convex with respect to $\alpha$, hence
\begin{equation}
\frac{\partial f}{\partial \alpha} \Big\vert_{\pmb{w} = \pmb{w}^{[m]}}
=
- 2 (\pmb{B}\pmb{w}^{[m]})^H
(	\pmb{y}
	-
	\alpha
	\pmb{B}
	\pmb{w}^{[m]})
	=
	\pmb{0}
\end{equation}
which gives the optimal solution to update $\alpha^{[m+1]}$ as 
\begin{equation}
	\label{eq:MM-update-1}
	\alpha^{[m+1]}
	=
	\frac{(\pmb{B}\pmb{w}^{[m]})^H \pmb{y}}{\Vert \pmb{B}
	\pmb{w}^{[m]} \Vert^2}
\end{equation}
Now unlike \eqref{eq:MM-1}, we will first expand $f(\alpha^{[m+1]}, \pmb{w})$ appearing in \eqref{eq:MM-2} as 
\begin{equation}
\label{eq:MM-step-2-1}
	f(\alpha^{[m+1]}, \pmb{w})
	=
	\Vert 
	\pmb{y}
	-
	\alpha^{[m+1]}
	\pmb{B}
	\pmb{w}
	\Vert^2
	=
	\pmb{y}^H \pmb{y}
	-
	2\Real(\alpha^{[m+1]} \pmb{y}^H 
	\pmb{B}
	\pmb{w})
	+
	\vert \alpha^{[m+1]} \vert^2  \Vert \pmb{B}
	\pmb{w} \Vert^2 
\end{equation}
Since the last term is convex in $\pmb{w}$, we can majorize it as 
\begin{equation}
\label{eq:MM-step-2-2}
\begin{split}
	\vert \alpha^{[m+1]} \vert^2  \Vert \pmb{B}
	\pmb{w} \Vert^2 
	&=
	\vert \alpha^{[m+1]} \vert^2
	\pmb{w}^H (\pmb{B}^H  \pmb{B}) \pmb{w} \\ &
	\leq
	\vert \alpha^{[m+1]} \vert^2
	\Big( 
	\lambda_{\max}(\pmb{B}^H  \pmb{B}) \Vert \pmb{w} \Vert^2 + 2 \Real(\pmb{w}^H [\pmb{B}^H  \pmb{B} - \lambda_{\max}(\pmb{B}^H  \pmb{B}) \pmb{I}]\pmb{w}^{[m]}) \\ &
	+
	(\pmb{w}^{[m]})^H
	(\lambda_{\max}(\pmb{B}^H  \pmb{B}) \pmb{I} - \pmb{B}^H  \pmb{B})\pmb{w}^{[m]}
	\Big),
\end{split}
\end{equation}
where $\lambda_{\max}(\pmb{B}^H  \pmb{B})$ returns the maximum eigenvalue of $\pmb{B}^H  \pmb{B}$. Now,
majorizing equation \eqref{eq:MM-step-2-1} by \eqref{eq:MM-step-2-2}, we get
\begin{equation}
\label{eq:upper-bound-MM}
\begin{split}
	f(\alpha^{[m+1]}, \pmb{w})
	&\leq
	\pmb{y}^H \pmb{y}
	-
	2\Real(\alpha^{[m+1]} \pmb{y}^H 
	\pmb{B}
	\pmb{w})
	+
	\vert \alpha^{[m+1]} \vert^2
	\lambda_{\max}(\pmb{B}^H  \pmb{B}) \Vert \pmb{w} \Vert^2 
	\\
	&+  2  \vert \alpha^{[m+1]} \vert^2\Real(\pmb{w}^H [\pmb{B}^H  \pmb{B} - \lambda_{\max}(\pmb{B}^H  \pmb{B}) \pmb{I}]\pmb{w}^{[m]}) 
	\\ &+
	\vert \alpha^{[m+1]} \vert^2
	(\pmb{w}^{[m]})^H
	(\lambda_{\max}(\pmb{B}^H  \pmb{B}) \pmb{I} - \pmb{B}^H  \pmb{B})\pmb{w}^{[m]}
\end{split}
\end{equation}
According to the majorization-minimization, instead of minimzing $f(\alpha^{[m+1]}, \pmb{w})$ under $\pmb{w} \in \mathcal{P}^{NP}$, we minimize the upper bound of it in \eqref{eq:upper-bound-MM}. Ignoring terms that are independent of $\pmb{w}$ (in addition to ignoring the term $\vert \alpha^{[m+1]} \vert^2
	\lambda_{\max}(\pmb{B}^H  \pmb{B}) \Vert \pmb{w} \Vert^2$ as $\Vert \pmb{w} \Vert^2$ is constant under $\pmb{w} \in \mathcal{P}^{NP}$), we now have
\begin{equation}
 \label{eq:problem6}
\begin{aligned}
(\mathcal{A}):
\begin{cases}
\min\limits_{\pmb{w}}& 	
	-2\Real \Big\lbrace \pmb{w}^H \Big( (\alpha^{[m+1]})^*  
	\pmb{B}^H
	\pmb{y} - \vert \alpha^{[m+1]} \vert^2([\pmb{B}^H  \pmb{B} - \lambda_{\max}(\pmb{B}^H  \pmb{B}) \pmb{I}]\pmb{w}^{[m]}) \Big)  \Big\rbrace    \\
\textrm{s.t.}
 & \pmb{w} \in \mathcal{P}^{NP},
\end{cases}
\end{aligned}
\end{equation}
which can be solved in closed for as 
\begin{equation}
	\label{eq:MM-update-2}
	\pmb{w}^{[m+1]}
	=
	\exp
	\Big (j  
	\arg
	\big\lbrace
(\alpha^{[m+1]})^*  
	\pmb{B}^H
	\pmb{y} - \vert \alpha^{[m+1]} \vert^2([\pmb{B}^H  \pmb{B} - \lambda_{\max}(\pmb{B}^H  \pmb{B}) \pmb{I}]\pmb{w}^{[m]})
	\big\rbrace
	\Big)
\end{equation}
where $\arg(\pmb{x})$ returns a vector of the same size as $\pmb{x}$ whose $i^{th}$ entry is the argument (or phase) of the $i^{th}$ entry of $\pmb{x}$. Iterating over \eqref{eq:MM-update-1} and \eqref{eq:MM-update-2}, we get
\begin{align}
	\label{eq:MM-iter-1}
	\alpha^{[m+1]}
	&=
	\frac{(\pmb{B}\pmb{w}^{[m]})^H \pmb{y}}{\Vert \pmb{B}
	\pmb{w}^{[m]} \Vert^2} \\
	\label{eq:MM-iter-2}
	\pmb{w}^{[m+1]}
	&=
	\exp
	\Big (j  
	\arg
	\big\lbrace
(\alpha^{[m+1]})^*  
	\pmb{B}^H
	\pmb{y} - \vert \alpha^{[m+1]} \vert^2([\pmb{B}^H  \pmb{B} - \lambda_{\max}(\pmb{B}^H  \pmb{B}) \pmb{I}]\pmb{w}^{[m]})
	\big\rbrace
	\Big)	
\end{align}
As an initializer of $\pmb{w}^{[m]}$, we have used $\pmb{w}^{[0]} = \exp(j \arg(\pmb{z}))$ where $\pmb{z} \sim \mathcal{CN}(0,\pmb{I}_{PN})$. \\



\begin{figure}[!t]
\centering
\includegraphics[width=4.5in]{./actions01/HAD/HAD-beampattern}
\caption{The resulting beampattern at the output of the hybrid analog beamformer for $\kappa_{\tt{high}} = 0\dB$ and $\kappa_{\tt{low}} = -60\dB$.}
\label{fig:HAD-Beampattern}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=4.5in]{./actions01/HAD/g-theta}
\caption{Evaluation of the spatial fit $g(\theta)$ defined in equation \eqref{eq:spatial-term}.}
\label{fig:g-theta}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=4.5in]{./actions01/HAD/MM-solver}
\caption{The convergence behaviour of the majorization-minimization solver described in equations \eqref{eq:MM-iter-1} and \eqref{eq:MM-iter-2}.}
\label{fig:MM-solver}
\end{figure}


Now, we run a simulation to evaluate the effectiveness of the hybrid analog beamformer, where we specify $\kappa_{\tt{high}} = 0\dB$ and $\kappa_{\tt{low}} = -60\dB$, and the radar sector of interest is $\pmb{\Omega}_r = [\pmb{\Omega}_r^{\tt{low}},\pmb{\Omega}_r^{\tt{high}}]$, with $\pmb{\Omega}_r^{\tt{low}} = -30^\circ$ and $\pmb{\Omega}_r^{\tt{high}} = 30^\circ$. Subsequently, we run the proposed majorization-minimization solver given in \eqref{eq:MM-iter-1} and \eqref{eq:MM-iter-2}.


In Fig. \ref{fig:HAD-Beampattern}, we can see that the resulting beampattern at the output of the hybrid analog beamformer matches the power specified by $y(\theta)$, i.e. $\kappa_{\tt{low}} = -60\dB$ when $\theta \notin \pmb{\Omega}_r$, otherwise $0\dB$ when $\theta \in \pmb{\Omega}_r$. 


In Fig. \ref{fig:g-theta}, we study the spatial fit $g(\theta)$ defined in \eqref{eq:spatial-term}, and we see that not only are the gains matched as per Fig. \ref{fig:HAD-Beampattern}, but so are the steering vectors $y(\theta) \pmb{a}(\theta)$ so as the estimation algorithms for hybrid radar fusion can effectively work. 


In Fig. \ref{fig:MM-solver}, we study the convergence behaviour of the iterative solver presented in \eqref{eq:MM-iter-1} and \eqref{eq:MM-iter-2}. We can see that the algorithm converges after about $100$ iterations.


%\end{document}






















==> actions01/acknowledge.tex <==
The authors would like to thank the anonymous reviewers for their constructive comments, which contributed in improving the manuscript.
The authors acknowledge that simulations were done on NYU Abu Dhabi's HPC Jubail Cluster. 

==> actions01/complexity-1.tex <==
Herein we analyze the complexity of each step appearing in \textbf{Algorithm \ref{alg:alg1}}. Before we proceed, let $N_\theta$ be the grid size while maximizing with respect to $\theta$ (e.g. the maximization in \eqref{eq:user-aoa-update-eqn} and \eqref{eq:phase-two-update-target-aoa}). The complexity is analyzed as follows:
\begin{enumerate}
%	\item Computing the fused covariance matrix $\widehat{\pmb{R}} = \sum\limits_{k=0}^K \widehat{\pmb{R}}_k$ costs $\mathcal{O}(K N^2 )$ as $K$ additions of $N\times N$ is required.
	\item Note that the initialization phase of \textbf{Algorithm \ref{alg:alg1}} is of the same order of complexity as phase $2$ as it involves running the alternating projection method for $q$ targets. Phase $2$ is analyzed in item 4 herein.
	\item Phase $1$ is now analyzed. Notice that $\pmb{P}_{\pmb{A}(\widehat{\pmb{\Theta}}^{\tt{tar}}_{(p)})}^{\perp}$ is independent of $\theta$ and $k$ and so it is computed once, which costs $\mathcal{O}(q^2 N + q^3 + q N^2)$. Also the term $\pmb{P}_{\pmb{A}(\widehat{\pmb{\Theta}}^{\tt{tar}}_{(p)})}^{\perp}
	\widehat{\pmb{R}}_k
	\pmb{P}_{\pmb{A}(\widehat{\pmb{\Theta}}^{\tt{tar}}_{(p)})}^{\perp}$ can be computed once before searching $[\widehat{\theta}_k^{\tt{u}}]_{(p)}$. This computation costs $\mathcal{O}(N^3)$.
	Each $\theta$ evaluation in the maximization process consists of evaluating \eqref{eq:user-aoa-update-eqn}, which costs $\mathcal{O}(N^2)$. Therefore, the entire search evaluates $\mathcal{O}(N_\theta N^2)$. Note that the peak search was ignored as this process scales linearly, in the worst case, with $N_\theta$ and so it will be dominated by the term $N_\theta N^2$.
	Summing over all $k$ (except the computation of $\pmb{P}_{\pmb{A}(\widehat{\pmb{\Theta}}^{\tt{tar}}_{(p)})}^{\perp}$) we get $\mathcal{O}(q^2 N + q^3 + q N^2 + KN^3 + KN_\theta N^2)$. 
	\item Phase $2$ is now analyzed. Notice that the term $\pmb{P}_{\widehat{\pmb{A}}_{k,m}^{(p)}}^\perp$ is independent of $\theta$ but depends on $k$ and $m$. Similar to $\pmb{P}_{\pmb{A}(\widehat{\pmb{\Theta}}^{\tt{tar}}_{(p)})}^{\perp}$, it costs $\mathcal{O}(q^2 N + q^3 + q N^2)$. Summing over all $K$, this means that computing all $\pmb{P}_{\widehat{\pmb{A}}_{k,m}^{(p)}}^\perp$ costs 
	$\mathcal{O}(q^2 K N + q^3 K + q K N^2)$.
	 Furthermore, calculating the terms $\pmb{P}_{\widehat{\pmb{A}}_{k,m}^{(p)}}^\perp \widehat{\pmb{R}}_k   \pmb{P}_{\widehat{\pmb{A}}_{k,m}^{(p)}}^\perp$ costs $\mathcal{O}(N^3)$. Summing over all $K$ will cost $\mathcal{O}(KN^3)$. Now, each $\theta$ evaluation in the maximization process consists of computing \eqref{eq:phase-two-update-target-aoa}, which costs $\mathcal{O}(KN^2)$. So, the whole search evaluates $\mathcal{O}(N_\theta K N^2)$. Summing over all $q$, we get $\mathcal{O}(qN_\theta K N^2 + q^3 K N + q^4 K + q^2 K N^2 + qKN^3)$.
\end{enumerate}
Assuming phase $1$ and phase $2$, as well as the initializer, iterate a total amount of $P_{\tt{iter}}$ times, and noting that phase $2$ dominates phase $1$, the total complexity of \textbf{Algorithm \ref{alg:alg1}} is
\begin{equation}
	T_1 = \mathcal{O}\Big(P_{\tt{iter}}(qN_\theta K N^2 + q^3 K N + q^4 K + q^2 K N^2 + qKN^3 ) \Big)
\end{equation}  
where we have ignored terms of lower orders. 










==> actions01/complexity-2.tex <==
Herein we analyze the complexity of each step appearing in \textbf{Algorithm \ref{alg:alg2}}. As we did when analyzing the complexity of \textbf{Algorithm \ref{alg:alg1}}, we let $N_\theta$ be the grid size while performing peak searches (e.g. during the maximization of $g_k(\theta)$ and when obtaining the $q$ strongest peaks in $h^{-1}(\theta)$ following  \eqref{eq:phase-two-Theta}). The complexity is analyzed as follows:
\begin{enumerate}
	\item Obtaining the noise subspace $\widehat{\pmb{U}}_{N,0}$ following \eqref{eq:EVD-on-sample-covariance-matrix} requires an \ac{EVD} of $\widehat{\pmb{R}}_0$, which costs $\mathcal{O}(N^3)$.
	\item Computing $\widehat{\pmb{P}}_0^{\perp}$ requires $\mathcal{O}(N^2(N-q))$.
 	\item For phase $1$, each $k$ iteration consists of   
\begin{enumerate}
	\item Obtain $\widehat{\bar{\pmb{R}}}_k 
$ using equation \eqref{eq:estimated-projected-covariance-phase-one}, requires multiplying $\widehat{\pmb{P}}_0^{\perp}$ with $\widehat{\pmb{R}}_k$, which costs $\mathcal{O}(N^3)$.

	\item The \ac{SVD} operation in \eqref{eq:the-first-svd} aiming at extracting $\pmb{v}_{S,k}$ costs $\mathcal{O}(N^3)$.
	\item Estimating $\widehat{\theta}_k^{\tt{u}}$ through maximizing via \eqref{eq:first-thetak-spectrum} can be achieved by first computing the term which is independent of $\theta$, namely, $\big[
	\pmb{v}_{S,k}
	\big(
	\pmb{v}_{S,k}^H
	\pmb{P}_0^{\perp}
	\pmb{v}_{S,k}
	\big)^{-1}
	\pmb{v}_{S,k}^H
	\pmb{P}_0^{\perp} - \pmb{I}_N \big]$, which costs costs $\mathcal{O}(N^3)$. Each evaluation of $\theta$ requires $\mathcal{O}(N^2)$. Summing over the entire grid size, this step costs $\mathcal{O}(N_\theta N^2 + N^3)$.
	
	\item Evaluating $\widehat{\pmb{Q}}_k^{\perp}$, for a give $\widehat{\theta}_k^{\tt{u}}$ utilizing \eqref{eq:Qk-projector-matrix} costs $\mathcal{O}(N^2)$.
	\item Calculating $\widehat{\pmb{S}}_k$ by applying \eqref{eq:computing-SK-proj} costs $\mathcal{O}(N^3)$. 
	\item The \ac{SVD} operation in \eqref{eq:obtaining-VSK-thru-Sk} costs $\mathcal{O}(N^3)$.
\end{enumerate}	
Summing phase $1$ over all $K$, the computational complexity of this Phase $1$ per iteration is dominated by $\mathcal{O}(KN_\theta N^2 + KN^3)$.

\item For phase $2$, we have to evaluate the peaks of $h^{-1}(\theta)$ followed by an orthogonal projector update of $\widehat{\pmb{P}}_0^{\perp}$. The complexities per iteration are as follows:
 
\begin{enumerate}
	\item For each $\theta$, the computation of $h(\theta)$ in \eqref{eq:h-theta-expression-for-algo-2} involves the computation of $ \Vert
\widehat{\pmb{U}}_{N,0}^H
	\pmb{a}(\theta) 
\Vert^2$ which costs $\mathcal{O}(N(N-q))$, followed by the computation of $\widehat{\pmb{V}}_{S,k}(\widehat{\pmb{Q}}_k^{\perp}
	\widehat{\pmb{V}}_{S,k})^+ 
	\widehat{\pmb{Q}}_k^{\perp}$ which costs $\mathcal{O}(qN^2 + q^2 N + q^3 + N^3)$, and is computed once per $k$ before grid evaluation. 
	Therefore, summing over all $K$, the computations of all $\widehat{\pmb{V}}_{S,k}(\widehat{\pmb{Q}}_k^{\perp}
	\widehat{\pmb{V}}_{S,k})^+ 
	\widehat{\pmb{Q}}_k^{\perp}$ over all $k$ costs $\mathcal{O}(KqN^2 + Kq^2 N + Kq^3 + KN^3)$.
	The evaluation of $\sum_{k=1}^K
 \Vert \widehat{\pmb{V}}_{S,k}(\widehat{\pmb{Q}}_k^{\perp}
	\widehat{\pmb{V}}_{S,k})^+ 
	\widehat{\pmb{Q}}_k^{\perp}
	\pmb{a}(\theta) - \pmb{a}(\theta) \Vert^2$ costs $\mathcal{O}(KN^2)$
	In short, the dominating terms of this step is $\mathcal{O}(N_\theta K N^2 + KqN^2 + Kq^2 N + Kq^3 + KN^3) $.
	\item Update $\widehat{\pmb{P}}_0^{\perp}$ costs $\mathcal{O}(q^2 N + q^3 + q N^2)$.
\end{enumerate}
Therefore, the computational complexity of Phase $2$ per iteration is dominated by $\mathcal{O}(N_\theta K N^2 + KqN^2 + Kq^2 N + Kq^3 + KN^3) $.
As the algorithm iterates between the two phases, we assume that the total number of iterations of $P_{\tt{iter}}$, which is assumed to be the same as \textbf{Algorithm \ref{alg:alg1}}. This is a reasonable assumption as per our simulations in Fig. \ref{fig:iterations} in the revised manuscript. The total complexity of \textbf{Algorithm \ref{alg:alg2}} is
\begin{equation}
	T_2 = \mathcal{O}\Big(P_{\tt{iter}}(
	N_\theta K N^2 + KqN^2 + Kq^2 N + Kq^3 + KN^3
	) \Big)
\end{equation} 

\end{enumerate}

==> actions01/complexity-compare.tex <==
In summary, we observe that $\frac{T_1}{T_2} \simeq \mathcal{O}(q)$.

==> actions01/direction-Tx-BFing-MIMO-response-item.tex <==
\begin{itemize}
	\item \textcolor{darkgreen}{The \ac{DFRC} \ac{BS} is now assumed to have $N_t$ transmit antennas dedicated for direction beams. For that, we added the following text in the beginning of Section \ref{sec:system-model}} 
	
	\textcolor{darkgreen}{We have also modified equation \eqref{eq:tx-OFDM-DL} in the revised manuscript to adapt for the multi-antenna case as follows}
	\begin{equation*}
		\input{equations-reuse/req12.tex}
	\end{equation*}
	\input{actions01/define-f.tex}
	
	
	
	\item \textcolor{darkgreen}{The above item also has a direct impact on the echo return of the \ac{DL} signal, as now each target explored by the \ac{DFRC} \ac{BS} (i.e. within $\Phi_0$) is also parameterized in terms of its \ac{AoD}. However, due to the mono-static assumption at the \ac{DFRC} \ac{BS}, the \ac{AoA} of the target is also its \ac{AoD}. To this end, the following text has been added on top of equation \eqref{eq:channel-DL-echo}  in the revised manuscript}\\
	\input{actions01/monostatic.tex}

	
	 \textcolor{darkgreen}{The following modification of equation \eqref{eq:rx-OFDM-echo} has been done}
	\begin{equation*}
		\input{equations-reuse/req1.tex}
	\end{equation*}
	\textcolor{darkgreen}{We have also defined $\pmb{a}_t(\theta)$ within the text below equation \eqref{eq:channel-DL-echo}, where the \ac{DL} echo channel has been introduced, and mentioned that the \ac{AoD} and \ac{AoA} are the same, thanks to mono-static configuration:\\}
	\input{actions01/define-at.tex}


	\item \textcolor{darkgreen}{As a result of introducing echo expression in equation \eqref{eq:rx-OFDM-echo}, equation \eqref{eq:sample-rx-OFDM} will also account for $\pmb{f}$, more precisely, in its first term as follows}
		\begin{equation*}
		\input{equations-reuse/req3.tex}
		\end{equation*}
			
	\item \textcolor{darkgreen}{Also, the frequency domain representation in equation \eqref{eq:DL-after-equalization} in the revised manuscript becomes}
	\begin{equation*}
		\input{equations-reuse/req4.tex}
	\end{equation*}
	
	\item \textcolor{darkgreen}{We have added Section \ref{sec:directional-beams} to discuss possible optimization problems in order to form directional beams for sensing and communications. The following is the content of the Section \ref{sec:directional-beams}:\\}
	\input{actions01/beamdirectional-section.tex}
\end{itemize}

==> actions01/discussion-section.tex <==
%% change to 
Even though transmit directional beamforming can amplify signal returns in certain radar regions, i.e. $\pmb{\Omega}_r$, for the mono-static \ac{DFRC} \ac{BS} operation, receive beamforming is also a necessary component for the \ac{HRF}. Indeed, the scattered signals from the target are generally orders of magnitude weaker than the direct \ac{LoS} \ac{UL} signal from the users, which in turn leads to an unreasonable high dynamic range of the \ac{ADCs} at the \ac{DFRC} \ac{BS}. 
This discrepancy in power between the scattered and \ac{LoS} components can be resolved in the analog domain by introducing hybrid analog beamformers before \ac{ADCs} so as to boost scattered returns within $\pmb{\Omega}_r$. In that way, the echo returns and the \ac{LoS} are power compatible. 
Regarding distances, targets that are far from the users can still yield high gains if they are sufficiently close to the \ac{DFRC} \ac{BS} \cite{pegoraro2023jump}. 
Hybrid analog beamforming design tailored for \ac{HRF} is left for future work.	

==> actions01/recover-UL-signals-response-comment.tex <==
For \ac{UL} communications, we can regard the direct-paths, along with the mixed reflected echoes as the channel matrix, which is used "as is" for equalization and later demodulation. 
Assuming the transmitted \ac{OFDM} symbol from the single-antenna $k^{th}$  user in the \ac{UL} is followed by an information embedded payload signal, i.e.
\begin{equation}
	s^{\tt{data}}_{k,\ell}(t) = 
	\sum\limits_{m \in \mathcal{C}_k }
	u_{m,k}^{(\ell)} \exp(j 2 \pi m \Delta_f t )
	\Pi(t- \ell T),
\end{equation}
where $u_{m,k}^{(\ell)} $ are modulated data belonging to a certain constellation. They are unknown to the \ac{DFRC} \ac{BS}. 
Passing $s^{\tt{data}}_{k,\ell}(t)$ through the $k^{th}$ \ac{UL} channel, the received signal at the \ac{DFRC} \ac{BS} is written as 
\begin{equation}
	\label{eq:rx-OFDM-payload}
	p_{n,\ell}(t) 
	=
	\sum\limits_{k=1}^K
	p_{n,\ell,k}^{\tt{UL}}(t)
	+
	w_{n,\ell}^{\tt{data}}(t),
\end{equation}
where we have assumed, for simplicity, that the \ac{BS} is not performing its downlink tasks in this time slot (i.e. only listening to \ac{UL} data), where 
\begin{equation}
\begin{split}
	p_{n,\ell,k}^{\tt{UL}}(t) 
	=
	\gamma_{0,\ell,k}^{\tt{u}}
	a_n(\theta_k^{\tt{u}})
	s^{\tt{data}}_{k,\ell}(t-\tau_k^{\tt{u}}) +
	\sum\limits_{i\in\Phi_k} 
	\gamma_{i,\ell,k}^{\tt{tar}} % this contains doppler
	a_n(\theta_i^{\tt{tar}})
	s^{\tt{data}}_{k,\ell}(t - \phi_{k,i}),
\end{split}
\end{equation} 
Sampling at $s \triangleq s \frac{T}{M}$, and following the same steps as equations \eqref{eq:sample-rx-OFDM} and \eqref{eq:DFT-formula} in the updated manuscript, we can write
\begin{equation}
	Y^{\tt{data}}_{n,\ell,m,k}
	=
	P_{n,\ell,m} \Big\vert_{m \in \mathcal{C}_k}, \quad 
	k = 1 \ldots K
\end{equation}
where $P_{n,\ell,m}
	=
	\frac{1}{M}
	\sum\limits_{s=0}^{M-1}
	p_{n,\ell}[s] 
	\exp\big(-j 2 \pi  \frac{m  s}{M} \big).$ The signal in frequency domain can be expressed as 
\begin{equation}
\begin{split}
	Y^{\tt{data}}_{n,\ell,m,k}
	=
	u_{m,k}^{(\ell)}
	\Big(		
	c_m(\tau_k^{\tt{u}})
	\gamma_{0,\ell,k}^{\tt{u}}
	a_n(\theta_k^{\tt{u}}) 
	+
	\sum\limits_{i \in \Phi_k} 
	c_m(\phi_{k,i})
	\gamma_{i,\ell,k}^{\tt{tar}} % this contains doppler
	a_n(\theta_i^{\tt{tar}})
	\Big) 
	+
	W^{\tt{data}}_{n,\ell,m,k}= 
	u_{m,k}^{(\ell)}
	\bar{Y}_{n,\ell,m,k}
	+
	W^{\tt{data}}_{n,\ell,m,k}, \\
\end{split}
\end{equation}
and from equation \eqref{eq:UL-after-equalization} in the updated manuscript, we have that $	Y_{n,\ell,m,k} =		\bar{Y}_{n,\ell,m,k} + W_{n,\ell,m,k}$, where $\bar{Y}_{n,\ell,m,k} = 	c_m(\tau_k^{\tt{u}})
	\gamma_{0,\ell,k}^{\tt{u}}
	a_n(\theta_k^{\tt{u}}) 
	+
	\sum\limits_{i \in \Phi_k} 
	c_m(\phi_{k,i})
	\gamma_{i,\ell,k}^{\tt{tar}} 
	a_n(\theta_i^{\tt{tar}})$. As we have a common channel, we can use $Y_{n,\ell,m,k}$ as a channel estimation and pass it from the training phase to the payload phase for equalization and demodulation. A schematic is shown in Fig. \ref{fig:timing-diagram}.
\begin{figure}[t]		
	\centering
\includegraphics[width=0.75\linewidth]{./actions01/timing-diagram.pdf}
	\caption{\textcolor{darkgreen}{Timing diagram to show the channel passed from the training phase to the data demodulation phase to decode the payload.}}
	\label{fig:timing-diagram}
\end{figure}
However, since the hybrid radar fusion improves the \ac{MSE} performance on $\pmb{\Theta}^{\tt{u}}$ and $\pmb{\Theta}^{\tt{tar}}$, we can use those estimates to aid parameterized channel reconstruction (i.e. reconstructing the channel based on the model). But, this method would require us to obtain additional estimates such as the delays, dopplers and gains. In the previous item, we described a "computational unfriendly" way of doing so, in the presence of synchronization errors. Future work will address this point, where we propose efficient and reliable estimators on the delays, dopplers and gains. Therefore, given all estimates of AoA, gain, delay and dopplers, we can reconstruct the channel and have an overall better channel estimate.

%If we expand equation \eqref{eq:DFT-formula} in the revised version, we have
%\begin{equation}
%		R_{n,\ell,m}
%		=
%		b_{m,k}^{(\ell)}
%		\Bigg(
%	\underbrace{c_m(\tau_k^{\tt{u}})
%	\gamma_{0,\ell,k}^{\tt{u}}
%	a_n(\theta_k^{\tt{u}})}_{\text{direct-path from user $k$}}
%	+
%	\underbrace{\sum\limits_{i=1}^q 
%	c_m(\phi_{k,i})
%	\gamma_{i,\ell,k}^{\tt{tar}} % this contains doppler
%	a_n(\theta_i^{\tt{tar}})}_{\text{uplink reflected echoes due to user $k$}}
%	\Bigg)\quad , m\in \mathcal{C}_k, \forall k \geq 1,
%\end{equation}
%and $R_{n,\ell,m}
%	=
%		b		_{m,0}^{(\ell)}
%		\sum\limits_{i=1}^q c_m(2\tau_i^{\tt{tar}})
%	\gamma_{i,\ell}^{\tt{tar}} 
%	a_n(\theta_i^{\tt{tar}}) $, for  $m \in \mathcal{C}_0$. 

%For the BS, how to independently recover uplink signals in direct-paths? Especially considering that theses components are mixed with the uplink reflected echoes.

%% Things to say:

% - A full frame design is expected in the followup paper.
% - The estimates yielded by the hybrid radar fusion can also be used for decoding.
% - 

==> actions01/reply-complexity.tex <==
\textbf{Reply Comment} \textcolor{darkgreen}{The authors would like to thank the reviewer for the comment. We provide below a thorough complexity comparison in terms of flops:}
\begin{itemize}
	\item 
	\textcolor{darkgreen}{\input{actions01/complexity-1.tex}}
	
	\item 
	\textcolor{darkgreen}{\input{actions01/complexity-2.tex}}
\end{itemize}
\textcolor{darkgreen}{\input{actions01/complexity-compare.tex}}

\textbf{Action:} \textcolor{darkgreen}{We have taken the following actions:}
\begin{itemize}
	\item \textcolor{darkgreen}{We have added Section \ref{sec:complexity-1} in the revised manuscript to summarize the computational complexity of \textbf{Algorithm \ref{alg:alg1}} by indicating that heaviest complexity is due to phase $2$. The following text has been added therein}\\
	\textcolor{blue}{\input{actions01/complexity-1-summary.tex}}
	
	\item \textcolor{darkgreen}{We have added Section \ref{sec:complexity-2} in the revised manuscript to summarize the computational complexity of \textbf{Algorithm \ref{alg:alg2}} by indicating that heaviest complexity is also due to phase $2$. The following text has been added therein}\\
	\textcolor{blue}{\input{actions01/complexity-2-summary.tex}}
\end{itemize}

==> actions01/reviewer2-response.tex <==
%The authors would like to thank the reviewer for the comment. We have placed the \ac{CRB} (dashed blue in Fig. \ref{fig:scene1_q3}, Fig. \ref{fig:scene2_q1}, and Fig. \ref{fig:scene2_q3} in the revised manuscript) for the general communication-centric mono-static, as well as bistatic only, ISAC model and shown in simulation that fusing information from \ac{UL} communication signals for radar sensing can improve the \ac{MSE} with increasing number of \ac{UL} communication users. 
%This guarantees that any traditional scheme for communication-centric mono-static ISAC will have an \ac{MSE} higher than the \ac{CRB} of the communication-centric mono-static ISAC. 
%Since we are mainly focusing on the estimation \ac{MSE} of target \ac{AoA}s, we focused our paper on proposing related algorithms that carefully combine \ac{UL} and \ac{DL} communication information to improve the target \ac{AoA} \ac{MSE}. On the other hand, since we observe that the \ac{MSE} improves by the proposed hybrid fusion model, we also would like to shed light on the merit of enhanced estimation: A better channel reconstruction mechanism can be designed based on the estimated target and user \ac{AoA}s, which in turn will have favorable impact on the equalization for \ac{UL} communications, which in return will improve \ac{UL} communication quality. The missing part however is the delay, doppler and gain estimation that is part of a future paper. More specifically, let us assume that a payload symbol is followed by the preamble in the form of 
%\begin{equation*}
%	s^{\tt{data}}_{k,\ell}(t) = 
%	\sum\limits_{m \in \mathcal{C}_k }
%	u_{m,k}^{(\ell)} \exp(j 2 \pi m \Delta_f t )
%	\Pi(t- \ell T),
%\end{equation*}
%where $u_{m,k}^{(\ell)} $ are modulated data belonging to a certain constellation. They are unknown to the \ac{DFRC} \ac{BS}. 
%Passing $s^{\tt{data}}_{k,\ell}(t)$ through the $k^{th}$ \ac{UL} channel, the received signal at the \ac{DFRC} \ac{BS} is written as 
%\begin{equation*}
%	p_{n,\ell}(t) 
%	=
%	\sum\limits_{k=1}^K
%	p_{n,\ell,k}^{\tt{UL}}(t)
%	+
%	w_{n,\ell}^{\tt{data}}(t),
%\end{equation*}
%For simplicity, we assume that when the \ac{UL} users transmit communication information, the \ac{DFRC} \ac{BS} does not participate in the \ac{DL}. Hence, the \ac{DFRC} \ac{BS} receives the \ac{UL} communication signal from $k^{th}$ user through direct (LoS) and bi-static link (echoes of targets) on the $k^{th}$ band $\mathcal{C}_k$,
%\begin{equation}
%\begin{split}
%	p_{n,\ell,k}^{\tt{UL}}(t) 
%	=
%	\gamma_{0,\ell,k}^{\tt{u}}
%	a_n(\theta_k^{\tt{u}})
%	s^{\tt{data}}_{k,\ell}(t-\tau_k^{\tt{u}}) +
%	\sum\limits_{i\in\Phi_k} 
%	\gamma_{i,\ell,k}^{\tt{tar}} % this contains doppler
%	a_n(\theta_i^{\tt{tar}})
%	s^{\tt{data}}_{k,\ell}(t - \phi_{k,i}),
%\end{split}
%\end{equation} 
%If we sample at regular intervals, i.e. $s \triangleq s \frac{T}{M}$, then similar to equations \eqref{eq:sample-rx-OFDM} and \eqref{eq:DFT-formula} in the updated manuscript, we have
%\begin{equation}
%	Y^{\tt{data}}_{n,\ell,m,k}
%	=
%	P_{n,\ell,m} \Big\vert_{m \in \mathcal{C}_k}, \quad 
%	k = 1 \ldots K
%\end{equation}
%where $P_{n,\ell,m}
%	=
%	\frac{1}{M}
%	\sum\limits_{s=0}^{M-1}
%	p_{n,\ell}[s] 
%	\exp\big(-j 2 \pi  \frac{m  s}{M} \big).$ The received frequency domain signal is 
%\begin{equation}
%\label{eq:communication-payload}
%\begin{split}
%	Y^{\tt{data}}_{n,\ell,m,k}
%	=
%	u_{m,k}^{(\ell)}
%	\Big(		
%	c_m(\tau_k^{\tt{u}})
%	\gamma_{0,\ell,k}^{\tt{u}}
%	a_n(\theta_k^{\tt{u}}) 
%	+
%	\sum\limits_{i \in \Phi_k} 
%	c_m(\phi_{k,i})
%	\gamma_{i,\ell,k}^{\tt{tar}} % this contains doppler
%	a_n(\theta_i^{\tt{tar}})
%	\Big) 
%	+
%	W^{\tt{data}}_{n,\ell,m,k},
%\end{split}
%\end{equation}
%The hybrid radar fusion improves the \ac{MSE} performance on $\pmb{\Theta}^{\tt{u}}$ and $\pmb{\Theta}^{\tt{tar}}$. Therefore, we can make use of these estimates to construct the channel for communication tasks, i.e. to equalize the channel in equation \eqref{eq:communication-payload} herein. The missing components for now are the doppler, gain and delay to construct such a channel, which is an aspect of a follow-up paper. Fig. \ref{fig:block-diagram} herein depicts a block diagram to show how the output of hybrid radar fusion can feed the equalization process for communications.
%\begin{figure}[t]		
%	\centering
%\includegraphics[width=0.75\linewidth]{./actions01/block-diagram-decoding.pdf}
%	\caption{\textcolor{darkgreen}{Block diagram of a communication-centric \ac{ISAC} \ac{DFRC} \ac{BS} making use of hybrid radar fusion.}}
%	\label{fig:block-diagram}
%\end{figure}


















%
%
%Second: Data rate or Estimation
%======
%This is estimation because comm-centric, it’s not about communication performance. %If you want to add other stuff, add it - but as new paragraph.
%
%Reformulate some CRB related things for monostatic and bistatic put in blue.


%
%First Part
%=======

%We did compare with other schemes in terms of CRB in this figure and this figure.
%Include more details about his question. 
The authors would like to thank the reviewer for the comment.
We compared with other schemes, such as general communication-centric mono-static and communication-centric bi-static \ac{ISAC}, in terms of their \ac{CRB}. 
Hybrid radar fusion's \ac{CRB} is lower than that of communication-centric mono-static and bi-static.
In specific, the hybrid radar fusion \ac{CRB} is given in equation \eqref{eq:HRF-CRB} in the manuscript, i.e.
\begin{equation*}
	\CRB(\pmb{\Theta}^{\tt{tar}}) = \frac{\sigma^2}{2}
	\Big(
    \sum\nolimits_{k=0}^K
	\sum\nolimits_{\ell=0}^{\bar{L}_k}
	\pmb{S}_k \pmb{F}_{k,\ell} \pmb{S}_k^T
	\Big)^{-1},
\end{equation*}
The mono-static \ac{CRB} accounts only for the \ac{DL} term for (i.e. $k = 0$), namely
\begin{equation*}
	\CRB_{\tt{mono-static}}(\pmb{\Theta}^{\tt{tar}}) = \frac{\sigma^2}{2}
	\Big(
	\sum\nolimits_{\ell=0}^{\bar{L}_0}
	\pmb{S}_0 \pmb{F}_{0,\ell} \pmb{S}_0^T
	\Big)^{-1},
\end{equation*}
and the bi-static \ac{CRB} accounts only for the bi-static terms $k = 1 \ldots K$, namely
\begin{equation*}
	\CRB_{\tt{bi-static}}(\pmb{\Theta}^{\tt{tar}}) = \frac{\sigma^2}{2}
	\Big(
    \sum\nolimits_{k=1}^K
	\sum\nolimits_{\ell=0}^{\bar{L}_k}
	\pmb{S}_k \pmb{F}_{k,\ell} \pmb{S}_k^T
	\Big)^{-1},
\end{equation*}
We have placed the mono-static \ac{CRB} (dashed blue) and bi-static \ac{CRB} (dashed black) in Fig. \ref{fig:scene1_q1}, Fig. \ref{fig:scene1_q3}, Fig. \ref{fig:scene2_q1}, and Fig. \ref{fig:scene2_q3} in the revised manuscript.

%Say monostatic doesn’t behave well because this and this 
%Bistatic which is this and this doesn’t behave well.
In the simulation corresponding to Fig. \ref{fig:scene1_q1} in the updated manuscript, we observe that for both $N=5$ and $N = 10$ cases, the \ac{CRB} of the mono-static and bi-static are very close. In fact, the hybrid radar fusion \ac{CRB} for only $K = 1$ user, improves the \ac{MSE} by nearly $5\dB$. In this figure as well, we have included a zoom-in sub-plot to show that the mono-static and bi-static configurations coincide in terms of \ac{CRB}. Furthermore, for the simulations corresponding to Fig. \ref{fig:scene1_q3}, we can notice that for the case of $N = 5$ antennas, the \ac{CRB} for $K = 1$ of hybrid radar fusion improves that of the mono-static by $5 \dB$, whereas there is a $10\dB$ gap between the mono-static and bi-static cases. On the other hand, for $N = 10$ antennas, we see that the bi-static \ac{CRB} approaches that of the mono-static. However, the single-user hybrid radar fusion improves by $4\dB$. Moreover, the simulations corresponding to Fig. \ref{fig:scene2_q1}, we can observe that the \ac{CRB} for single-user of hybrid radar fusion, which improves the mono-static \ac{CRB} by $1.8\dB$, and improves the bi-static by $4.8\dB$. In addition, by referring to Fig. \ref{fig:scene2_q3} for $N = 10$ antennas, we observe that the hybrid radar fusion \ac{CRB} for $K=1$ is $1.3\dB$ lower than the mono-static case, and can further improve the bi-static configuration by $5\dB$. Therefore, in general the hybrid radar fusion has the full potential to improve mono-static and bi-static communication-centric \ac{ISAC} systems. In addition, within the literature, we are not aware of any other benchmarks that we can compare with, because this hybrid radar fusion is a newly introduced concept.


%Second: Data rate or Estimation
%======
%This is estimation because comm-centric, it’s not about communication performance. %If you want to add other stuff, add it - but as new paragraph.
In addition to the \ac{CRB}, we would also like to clarify that the hybrid radar fusion has the full capability to enhance \ac{MSE} performance in the context of communication-centric systems. The communication counterpart of the system remains fully functional, as sensing in this case comes as an add-on, which leverages and exploits an already existing communication infrastructure. 





















==> actions01/summary-of-actions.tex <==
In light of the reviewers comments, we summarize our action items as follows:
\begin{itemize}
	\item We have adapted our system model and parts of the algorithms for the more general case, where the users and \ac{BS} explore different targets, reflected by the sets of $\Phi_0 \ldots \Phi_K$.
	\item We have not only extended the hybrid radar fusion system model to multiple transmit antennas, which allows us to perform transmit beamforming to further enhance \ac{DL} detection and radar performance, but we have also dedicated a section describing how hybrid radar fusion can for directional beams via two optimization frameworks. Each optimization problem has its own characteristics, which are clarified and discussed.
	\item Receive beamforming through hybrid analog beamforming is discussed only in this response letter for lack of space. This receive beamformer is desirable because it preserves the receive steering vector which will further be exploited by the hybrid radar fusion algorithms. We have given simulations in this response letter to highlight the potential of a solver that can optimize for the phase shifts that are placed before the \ac{LNA} and \ac{ADC}. These simulations include convergence behavior of the method as well as the obtained beampattern. The analog part performs receive beamforming over a radar sector of interest (where radar sensing takes place). This has the merit of amplifying weak signals up to a desired power level (and in particular to the power level of \ac{LoS} components), which then drastically lowers the dynamic range required by \ac{ADC} converters. 
	\item We have explicitly characterized the \ac{UL} and \ac{DL} channels as part of the hybrid radar fusion system model. We have also explicitly mentioned the signal and double-path loss gains for each of the \ac{UL} and \ac{DL} channels as function of distances, antenna gains, wavelength and \ac{RCS}. 
	\item The system settings, such as distances, have been evaluated in the simulation section.
	\item We have mentioned that indeed the estimator of $\pmb{X}_k$ is not the exact \ac{ML} estimator, but a relaxed version of it. We have justified this due to our interest in only the \ac{AoA} estimates of users and targets. We have also chosen to relax $\pmb{X}_k$ as an arbitrary matrix due to the many parameters it includes (distances, gains, doppler and delays). 
	\item We have included a detailed computational complexity analysis of \textbf{Algorithm \ref{alg:alg1}} and \textbf{Algorithm \ref{alg:alg2}} in this response letter. We have included a summary of the computational complexity analysis in the revised manuscript due to lack of space.
	\item We have highlighted that the hybrid radar fusion performs better than communication-centric mono-static, as well as bistatic, \ac{ISAC} by depicting the \ac{CRB} of both mono-static and bi-static versus the hybrid radar fusion with increasing \ac{UL} communication users. We have also discussed the possibility of using the estimates in an attempt to reconstruct the channel for equalization, as part of the \ac{UL} communication tasks. Since the hybrid is a new scheme, there is no other benchmark about the hybrid we could compare with except the classical mono-static and bi-static.
	\item We have mentioned that the proposed hybrid radar fusion model falls under the category of communication-assisted sensing, where our main interest lies in the estimation of target \ac{AoA}s, where we exploit a well-established communication infrastructure. Here, sensing is an add-on given to a communication system.
	\item We have fully described a methodology, in this response letter, on how synchronization can be established on the bi-static part of the hybrid radar fusion model. More specifically, we have further estimated matrices $\pmb{X}_k$ and under some optimization fitting methods, we have jointly estimated the distances and the offsets arising from misalignment of clock oscillators between the \ac{UL} users and the \ac{DFRC} \ac{BS}. We have simulated results based on the achieved \ac{NMSE} of the time offset, frequency offset and the estimated distance of the user. Due to lack of space, and the computational complexity of the method, we leave this method as part of future work.
	\item We have highlighted that the steering response, in general, is indeed a function of the frequency, as well as the angle. We have justified our narrowband assumption, which in turn enables us to approximate the steering response as a function of the angle and the carrier frequency, thus neglecting the beam-squint effect.
	\item We have included the case of moving targets, through the introduction of doppler frequencies as part of the sensing parameters. The doppler frequencies are now made explicit in our hybrid radar fusion model. Similar to the delays, the doppler frequencies are absorbed within the matrices $\pmb{X}_k$, which we treat as nuissance parameters. Hence, this shows that the hybrid radar fusion method can still work regardless of static or moving targets.
	\item We have justified how "Algorithm 1 with prior knowledge" can obtain the knowledge of user \ac{AoAs} in practice. Namely, this knowledge can be obtained via \ac{GNSS} or by tracking via a two-stage approach, where in stage one, \textbf{Algorithm \ref{alg:alg1}} or \textbf{Algorithm \ref{alg:alg2}} is executed without prior knowledge of user positions, then in stage two, the user \ac{AoAs} can be used as prior knowledge for \textbf{Algorithm \ref{alg:alg1}}.
	\item We have corrected all reference formats. The format of the references are now consistent with the \ac{IEEE} format, thanks to the usage of the BibTeX reference management software.
	\item We have described how the \ac{DFRC} \ac{BS} can use the channel estimates to recover uplink signals, even though they are mixed with the echo signals for upcoming symbols carrying payload data.
	\item We have corrected some chaotic subscripts.
	\item We have shown in details, in this response letter, how the noise component will contain only the gaussian terms without inter-user interference arising from the last three terms of equation (7) in the first submission (now equation \eqref{eq:sample-rx-OFDM} in the updated manuscript). In short, this is due to the \ac{FDD} protocol followed in the paper, where each user transmits on its own band $\mathcal{C}_k$. Additionally, we have corrected an assumption by strengthening it to $\mathcal{C}_i \cap \mathcal{C}_j = \emptyset$ for all $i \neq j$. Lastly, and for simplicity, we have assumed that the preamble is an all-ones sequence so that the noise is \ac{AWGN}.
	\item Fig. 4 and Fig. 5 previously (now Fig. \ref{fig:scene2_q1} and Fig. \ref{fig:scene2_q3} in the updated manuscript) now contain a zoom-in subplot at the upper right region of the respective plots. 


\item We have summarized different parts to abide by the $16$ double-column single-spaced pages ($10$-point font size, 1-inch margin on all sides) including the title, names of the authors and our complete contact information, abstract, text, equations, figures, and all references, as indicated by the submission guidelines of the IEEE Transactions on Wireless Communications, effective July $1$, $2023$.
\end{itemize}


%	(Characterized channel + In order to reduce dynamic range requirements at the receiver, we consider a hybrid analog beamformer scheme where the reduced dynamic range comes at the price of spatial oversampling...)


%\textbf{Deleted Items:} We have deleted/resized the following items to respect the 15-page double column limit as per the submission guidelines:
%\begin{itemize}
%	\item deleted-item-01
%	\item deleted-item-02
%	\item deleted-item-03
%\end{itemize}

==> actions01/synchronization-action-item.tex <==
\textcolor{darkgreen}{We have added the following text below equation \eqref{eq:Xk-matrix-form} in the revised manuscript, with intentions to summarize what has been done in the \textbf{Reply Comment} of this comment.\\}
\input{actions01/synchronization-phrase.tex}



==> actions01/synchronization-response-comment.tex <==
\textcolor{darkgreen}{Definitely, synchronization between the DFRC BS and the different communication users is crucial, if the parameters of interest are the delays and/or the dopplers. 
In practice, and due to hardware impairments, there always exist time and frequency offsets between the users and the DFRC BS. In particular, this arises because of the the oscillator clocks of the unlocked (or unsynchronized) clocks between the DFRC BS and the communication users. 
Following \cite{zhang2021overview} (c.f. equation (2)), we can adapt our model, which leads to equation \eqref{eq:DL-after-equalization} (in the updated manuscript) which can be written in the following form
\begin{equation*}
	Y_{n,\ell,m}
	=
	\sum\limits_{i \in \Phi_0} c_m(2
	\tilde{\tau}_i^{\tt{tar}})
	\tilde{\gamma}_{i,\ell}^{\tt{tar}} % this contains doppler
	(\pmb{a}_t^T(\theta_i^{\tt{tar}}) \pmb{f})
	a_n(\theta_i^{\tt{tar}})
	+
	W_{n,\ell,m},
\end{equation*}
for $m \in \mathcal{C}_0$ and equation \eqref{eq:UL-after-equalization} in the updated manuscript  can be written as follows
\begin{equation*}
	Y_{n,\ell,m}
	=		
	c_m(\tilde{\tau}_k^{\tt{u}})
	\gamma_{0,\ell,k}^{\tt{u}}
	a_n(\theta_k^{\tt{u}}) 
	+
	\sum\limits_{i \in \Phi_k} 
	c_m(\tilde{\phi}_{k,i})
	\tilde{\gamma}_{i,\ell,k}^{\tt{tar}} % this contains doppler
	a_n(\theta_i^{\tt{tar}}) +
	W_{n,\ell,m},
\end{equation*}
for $m \in \mathcal{C}_k$ for all $k = 1\ldots K$, 
where 
$\tilde{\tau}_i^{\tt{tar}} = {\tau}_i^{\tt{tar}} + \delta^\tau_k$, 
$\tilde{\tau}_k^{\tt{u}} = {\tau}_k^{\tt{u}} + \delta^\tau_k$,
$\tilde{\phi}_{k,i} = {\phi}_{k,i} + \delta^\tau_k$,
$\tilde{\gamma}_{i,\ell}^{\tt{tar}} = g_{i}^{\tt{tar}} e^{j 2 \pi \ell T (f_{D,i} + \delta^f_k) }$,
and 
$\tilde{\gamma}_{i,\ell,k}^{\tt{tar}} = g_{i,k}^{\tt{tar}} e^{j 2 \pi \ell T (f_{D,i} + \delta^f_k)}$
where $\delta^\tau_k$ and $\delta^f_k$ represent the time offset and frequency offset due to the oscillator drift between that of the \ac{DFRC} \ac{BS} and the $k^{th}$ user.
If a crystal oscillator deviates with $10$ppm, then the time offset can accumulate over $0.1$ms a deviation of 1 nanoseconds, which translates to $0.3$ meters, which can be dramatic for sensing. 
However, since our parameters of interest lie in the \ac{AoAs} of the targets and users, we can observe that the derived maximum likelihood estimator treats the offsets, along with delays, dopplers and gains as nuissance parameters. To show this, equations \eqref{eq:matrix-form-UL} and \eqref{eq:matrix-form-DL} in the updated manuscript are now in the form of 
\begin{equation*}
	\pmb{Y}_0
	= 
	\pmb{A}(\pmb{\Theta}^{\tt{tar}}_0)
	\tilde{\pmb{X}}_0
	+
	\pmb{W}_0,
\end{equation*}
and
\begin{equation*}
	\pmb{Y}_k
	= 
	\begin{bmatrix}
		\pmb{a}(\theta_k^{\tt{u}}) &		
		\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)
	\end{bmatrix}
	\tilde{\pmb{X}}_k + \pmb{W}_k, \quad k = 1 \ldots K.
\end{equation*}
where $\tilde{\pmb{X}}_k$ is given as 
\begin{equation}
	\label{eq:Xk-with-offsets}
	\tilde{\pmb{X}}_k
	=
	\begin{bmatrix}
		\tilde{\pmb{x}}_{1,p_1}^{(k)}
		,
		\ldots
		,
		\tilde{\pmb{x}}_{L_k,p_1}^{(k)}
		,
		\ldots
		,
		\tilde{\pmb{x}}_{1,p_{\vert \mathcal{C}_k\vert}}^{(k)}
		,
		\ldots
		,
		\tilde{\pmb{x}}_{L_k,p_{\vert \mathcal{C}_k\vert}}^{(k)}
	\end{bmatrix},
\end{equation}
and
 \begin{equation}
 \label{eq:xlmk1-offset}
 	\tilde{\pmb{x}}_{\ell,m}^{(k)}
 	=
 	\begin{cases}
 			\begin{bmatrix}
 		\tilde{\gamma}_{u_1^{(0)},\ell}^{\tt{tar}} c_m(2\tilde{\tau}_{u_1^{(0)}}^{\tt{tar}}) \\
 		 \vdots \\
 		 \tilde{\gamma}_{u^{(0)}_{\vert \Phi_0 \vert},\ell}^{\tt{tar}} c_m(2\tilde{\tau}_{u^{(0)}_{\vert \Phi_0 \vert}}^{\tt{tar}})
 	\end{bmatrix}
 	\in \mathbb{C}^{\vert \Phi_0 \vert \times 1}
 	, & k = 0 \\
 	\begin{bmatrix}
 	\gamma_{0,\ell,k}^{\tt{u}} c_m(\tilde{\tau}_k^{\tt{u}})
 	 \\
 		\tilde{\gamma}_{u_1^{(k)},\ell,k}^{\tt{tar}} c_m(\tilde{\phi}_{k,u_1^{(k)}}) \\
 		 \vdots \\
 		 \tilde{\gamma}_{u^{(k)}_{\vert \Phi_k \vert},\ell,k}^{\tt{tar}} c_m(\tilde{\phi}_{k,u^{(k)}_{\vert \Phi_k \vert}})
 	\end{bmatrix}
 	\in \mathbb{C}^{(\vert \Phi_k \vert+1) \times 1}
 	, & 1 \leq k \leq K.
 	\end{cases}
 \end{equation}
  Please note that the time offsets and frequency offsets are absorbed within the equation above, which means that there will be no impact on the AoA estimates. Hence equation \eqref{eq:ML-X} in the updated manuscript will contain the time/frequency offsets within, i.e.
 \begin{equation*}
	\widehat{\tilde{\pmb{X}}}_k
	=
	\big(
	\pmb{A}_k^H
	\pmb{A}_k
	\big)^{-1}
	\pmb{A}_k^H
	\pmb{Y}_k.
\end{equation*}
This also means that if we take a step further and estimate delays and dopplers, then we would have to either jointly estimate the time/frequency offset parameters, or pre-compensate for it. Assuming we are interested in the former, then one way to proceed is to reconstruct $\pmb{A}_k$ via the \ac{AoA} estimates obtained by \textbf{Algorithm \ref{alg:alg1}} or \textbf{Algorithm \ref{alg:alg2}}. More specifically, we use the estimates $\pmb{\Theta}^{\tt{tar}}_k$ and $\pmb{\Theta}^{\tt{u}}$ to construct an estimate of $\pmb{A}_k$ (denoted as $\widehat{\pmb{A}}_k$) with the aid of equation \eqref{eq:Ak-definition} in the updated manuscript. Then we can proceed in applying the above equation to obtain an estimate of ${\tilde{\pmb{X}}}_k$ as $\widehat{\tilde{\pmb{X}}}_k
	=
	\big(
	\widehat{\pmb{A}}_k^H
	\widehat{\pmb{A}}_k
	\big)^{-1}
	\widehat{\pmb{A}}_k^H
	\pmb{Y}_k$. 
	Next, one can fit the obtained $\widehat{\tilde{\pmb{X}}}_k$ via the model it follows in equation \eqref{eq:xlmk1-offset} herein, as follows
	\begin{equation}
	\label{eq:joint-offset-delay-doppler-estimation}
	\hat{\pmb{d}}^{\tt{tar}},
		\hat{\pmb{d}}^{\tt{u}},
		\hat{\pmb{d}},
		\hat{\pmb{f}}_D,
		\hat{\pmb{\sigma}}_{\tt{RCS}},
		\hat{\pmb{\delta}}^\tau,
		\hat{\pmb{\delta}}^f
		=
		\argmin_{		\pmb{d}^{\tt{tar}},
		\pmb{d}^{\tt{u}},
		\pmb{d},
		\pmb{f}_D,
		\pmb{\sigma}_{\tt{RCS}},
		\pmb{\delta}^\tau,
		\pmb{\delta}^f}
		\sum_{k=0}^K 
		 \Bigg\Vert
		\widehat{\tilde{\pmb{X}}}_k
		-
		\tilde{\pmb{X}}_k
		\Big(
		\pmb{d}^{\tt{tar}},
		\pmb{d}^{\tt{u}},
		\pmb{d},
		\pmb{f}_D,
		\pmb{\sigma}_{\tt{RCS}},
		{\delta}^\tau_k,
		{\delta}^f_k
		\Big)
		 \Bigg\Vert^2,
	\end{equation}
	where in the above we have made explicit that $\tilde{\pmb{X}}_k$ in equation \eqref{eq:Xk-with-offsets} herein depends on the distances (equivalently delays and gains), dopplers, RCS values, as well as time and frequency offsets. 
	 $\pmb{d}^{\tt{tar}}$ is a vector containing all target distances, i.e. ${\tau}^{\tt{tar}}_1 \ldots {\tau}^{\tt{tar}}_q$.
	The vector $\pmb{d}^{\tt{u}}$ is a vector containing all user distances, namely ${\tau}^{\tt{u}}_1 \ldots {\tau}^{\tt{u}}_K$. 
	The vector $\pmb{d}$ is a vector containing all user target-user distances. As a reminder, we have that $\phi_{k,i} = \frac{d_{k,i} + d_i^{\tt{tar}}}{c} = \tau_{k,i}+\tau^{\tt{tar}}_i$.
	The vector $\pmb{f}_D$ contains dopplers of all the targets.
	The vector $\pmb{\sigma}_{\tt{RCS}}$ contains all  target \ac{RCS} values. 
	The vectors $\pmb{\delta}^\tau,
		\pmb{\delta}^f$ contain all the $K$ time offsets and $K$ frequency offsets, respectively.
	The optimization problem in \eqref{eq:joint-offset-delay-doppler-estimation} herein is too complex to solve. Instead, we note that $\tilde{\pmb{x}}_{\ell,m}^{(k)}$ can be written in terms of its synchronized version as 
 \begin{equation}
 	\tilde{\pmb{x}}_{\ell,m}^{(k)}
 	=
 	{\pmb{x}}_{\ell,m}^{(k)}
 	 \exp(-j 2 \pi m \Delta_f \delta_\tau )
 	 \exp(j 2 \pi \ell T \delta_f)
 	 =
 	 {\pmb{x}}_{\ell,m}^{(k)}
 	 \exp(j 2\pi (-m \Delta_f \delta^\tau_k + \ell T \delta^f_k) ),
 \end{equation}
 where ${\pmb{x}}_{\ell,m}^{(k)}$ is obtained by setting $\delta^f_k$ and $\delta^\tau_k$ to zero in equation the expression of $\tilde{\pmb{x}}_{\ell,m}^{(k)}$ herein. 
 Using this, we can decouple the search per user while searching for $\delta^f_k$ and $\delta^\tau_k$.
 We experiment the estimator in \eqref{eq:joint-offset-delay-doppler-estimation} for $K = 1$ user and $q = 1$ target, where the user is placed at $\hat{d}_1^{\tt{u}} = 100$m away from the \ac{DFRC} \ac{BS}. 
 We set $\delta^f_1$ to $5$ppm, which corresponds to $\delta^f_1 = 120$KHz at $24$ GHz. 
 We set $\delta^\tau_1 = 0.3\mu$sec.
 In Fig. \ref{fig:NMSE-FO}, Fig. \ref{fig:NMSE-TO}, and Fig. \ref{fig:NMSE-distance}, we plot the \ac{NMSE} for all three parameters, which are defined as follows
 \begin{equation*}
	\NMSE(\hat{\delta}^f_1)
	=
	\frac{1}{E}
	\sum_{e = 1}^E
	\frac{\Vert \delta^f_1 - \hat{\delta}^f_1(e) \Vert^2}{\Vert \delta^f_1 \Vert^2},
 \end{equation*}
  \begin{equation*}
	\NMSE(\hat{\delta}^\tau_1)
	=
	\frac{1}{E}
	\sum_{e = 1}^E
	\frac{\Vert \delta^\tau_1 - \hat{\delta}^\tau_1(e) \Vert^2}{\Vert \delta^\tau_1 \Vert^2},
 \end{equation*}
   \begin{equation*}
	\NMSE(\hat{d}_1^{\tt{u}})
	=
	\frac{1}{E}
	\sum_{e = 1}^E
	\frac{\Vert {d}_1^{\tt{u}} - \hat{d}_1^{\tt{u}}(e) \Vert^2}{\Vert {d}_1^{\tt{u}}\Vert^2},
 \end{equation*}
 where $\hat{\delta}^f_1(e), \hat{\delta}^\tau_1(e),$ and $\hat{d}_1^{\tt{u}}$ are the estimated values of ${\delta}^f_1(e), {\delta}^\tau_1(e),$ and ${d}_1^{\tt{u}}$ at the $e^{th}$ monte carlo simulation, respectively, through the multi-dimensional search adopted in \eqref{eq:joint-offset-delay-doppler-estimation} herein.
 We can see that the method can give satisfying results for high \ac{SNR}, which has a positive effect on distance estimation as shown in Fig. \ref{fig:NMSE-distance}.
 In an ongoing paper, we intend to perform doppler and distance estimation by including the synchronization issue for the bistatic counterpart. We are currently preparing the paper that includes these topics.  
}

\textcolor{darkgreen}{We would have indeed liked to include this section, however since ToA and doppler is not our primary estimation focus in this paper, we will address synchronization issues in a follow-up paper.\\}

==> actions01/synchronization-response-comment2.tex <==
\textcolor{darkgreen}{Definitely, synchronization between the DFRC BS and the different communication users is crucial, if the parameters of interest are the delays and/or the dopplers. 
In practice, and due to hardware impairments, there always exist time and frequency offsets between the users and the DFRC BS. In particular, this arises because of the the oscillator clocks of the unlocked (or unsynchronized) clocks between the DFRC BS and the communication users. 
Following \cite{zhang2021overview} (c.f. equation (2)), we can adapt our model, which leads to equation \eqref{eq:DL-after-equalization} (in the updated manuscript) which can be written in the following form
\begin{equation*}
	Y_{n,\ell,m}
	=
	\sum\limits_{i \in \Phi_0} c_m(2
	\tilde{\tau}_i^{\tt{tar}})
	\tilde{\gamma}_{i,\ell}^{\tt{tar}} % this contains doppler
	(\pmb{a}_t^T(\theta_i^{\tt{tar}}) \pmb{f})
	a_n(\theta_i^{\tt{tar}})
	+
	W_{n,\ell,m},
\end{equation*}
for $m \in \mathcal{C}_0$ and equation \eqref{eq:UL-after-equalization} in the updated manuscript can be written as follows
\begin{equation*}
	Y_{n,\ell,m}
	=		
	c_m(\tilde{\tau}_k^{\tt{u}})
	\gamma_{0,\ell,k}^{\tt{u}}
	a_n(\theta_k^{\tt{u}}) 
	+
	\sum\limits_{i \in \Phi_k} 
	c_m(\tilde{\phi}_{k,i})
	\tilde{\gamma}_{i,\ell,k}^{\tt{tar}} % this contains doppler
	a_n(\theta_i^{\tt{tar}}) +
	W_{n,\ell,m},
\end{equation*}
for $m \in \mathcal{C}_k$ for all $k = 1\ldots K$, 
where 
$\tilde{\tau}_i^{\tt{tar}} = {\tau}_i^{\tt{tar}} + \delta^\tau_k$, 
$\tilde{\tau}_k^{\tt{u}} = {\tau}_k^{\tt{u}} + \delta^\tau_k$,
$\tilde{\phi}_{k,i} = {\phi}_{k,i} + \delta^\tau_k$,
$\tilde{\gamma}_{i,\ell}^{\tt{tar}} = g_{i}^{\tt{tar}} e^{j 2 \pi \ell T (f_{D,i} + \delta^f_k) }$,
and 
$\tilde{\gamma}_{i,\ell,k}^{\tt{tar}} = g_{i,k}^{\tt{tar}} e^{j 2 \pi \ell T (f_{D,i} + \delta^f_k)}$
where $\delta^\tau_k$ and $\delta^f_k$ represent the time offset and frequency offset due to the oscillator drift between that of the \ac{DFRC} \ac{BS} and the $k^{th}$ user.
If a crystal oscillator deviates with $10$ppm, then the time offset can accumulate over $0.1$ms a deviation of 1 nanoseconds, which translates to $0.3$ meters, which can be dramatic for sensing. 
However, since our parameters of interest lie in the \ac{AoAs} of the targets and users, we can observe that the derived maximum likelihood estimator treats the offsets, along with delays, dopplers and gains as nuissance parameters. To show this, equations \eqref{eq:matrix-form-UL} and \eqref{eq:matrix-form-DL} in the updated manuscript are now in the form of 
\begin{equation*}
	\pmb{Y}_0
	= 
	\pmb{A}(\pmb{\Theta}^{\tt{tar}}_0)
	\tilde{\pmb{X}}_0
	+
	\pmb{W}_0,
\end{equation*}
and
\begin{equation*}
	\pmb{Y}_k
	= 
	\begin{bmatrix}
		\pmb{a}(\theta_k^{\tt{u}}) &		
		\pmb{A}(\pmb{\Theta}^{\tt{tar}}_k)
	\end{bmatrix}
	\tilde{\pmb{X}}_k + \pmb{W}_k, \quad k = 1 \ldots K.
\end{equation*}
where $\tilde{\pmb{X}}_k$ is given as 
\begin{equation}
	\label{eq:Xk-with-offsets2}
	\tilde{\pmb{X}}_k
	=
	\begin{bmatrix}
		\tilde{\pmb{x}}_{1,p_1}^{(k)}
		,
		\ldots
		,
		\tilde{\pmb{x}}_{L_k,p_1}^{(k)}
		,
		\ldots
		,
		\tilde{\pmb{x}}_{1,p_{\vert \mathcal{C}_k\vert}}^{(k)}
		,
		\ldots
		,
		\tilde{\pmb{x}}_{L_k,p_{\vert \mathcal{C}_k\vert}}^{(k)}
	\end{bmatrix},
\end{equation}
and
 \begin{equation}
 \label{eq:xlmk1-offset2}
 	\tilde{\pmb{x}}_{\ell,m}^{(k)}
 	=
 	\begin{cases}
 			\begin{bmatrix}
 		\tilde{\gamma}_{u_1^{(0)},\ell}^{\tt{tar}} c_m(2\tilde{\tau}_{u_1^{(0)}}^{\tt{tar}}) \\
 		 \vdots \\
 		 \tilde{\gamma}_{u^{(0)}_{\vert \Phi_0 \vert},\ell}^{\tt{tar}} c_m(2\tilde{\tau}_{u^{(0)}_{\vert \Phi_0 \vert}}^{\tt{tar}})
 	\end{bmatrix}
 	\in \mathbb{C}^{\vert \Phi_0 \vert \times 1}
 	, & k = 0 \\
 	\begin{bmatrix}
 	\gamma_{0,\ell,k}^{\tt{u}} c_m(\tilde{\tau}_k^{\tt{u}})
 	 \\
 		\tilde{\gamma}_{u_1^{(k)},\ell,k}^{\tt{tar}} c_m(\tilde{\phi}_{k,u_1^{(k)}}) \\
 		 \vdots \\
 		 \tilde{\gamma}_{u^{(k)}_{\vert \Phi_k \vert},\ell,k}^{\tt{tar}} c_m(\tilde{\phi}_{k,u^{(k)}_{\vert \Phi_k \vert}})
 	\end{bmatrix}
 	\in \mathbb{C}^{(\vert \Phi_k \vert+1) \times 1}
 	, & 1 \leq k \leq K.
 	\end{cases}
 \end{equation}
  Please note that the time offsets and frequency offsets are absorbed within equation above, which means that there will be no impact on the AoA estimates. Hence equation \eqref{eq:ML-X} in the updated manuscript will contain the time/frequency offsets within, i.e.
 \begin{equation*}
	\widehat{\tilde{\pmb{X}}}_k
	=
	\big(
	\pmb{A}_k^H
	\pmb{A}_k
	\big)^{-1}
	\pmb{A}_k^H
	\pmb{Y}_k.
\end{equation*}
This also means that if we take a step further and estimate delays and dopplers, then we would have to either jointly estimate the time/frequency offset parameters, or pre-compensate for it. Assuming we are interested in the former, then one way to proceed is to reconstruct $\pmb{A}_k$ via the \ac{AoA} estimates obtained by \textbf{Algorithm \ref{alg:alg1}} or \textbf{Algorithm \ref{alg:alg2}}. More specifically, we use the estimates $\pmb{\Theta}^{\tt{tar}}_k$ and $\pmb{\Theta}^{\tt{u}}$ to construct an estimate of $\pmb{A}_k$ (denoted as $\widehat{\pmb{A}}_k$) with the aid of equation \eqref{eq:Ak-definition} in the updated manuscript. Then we can proceed in applying the above equation to obtain an estimate of ${\tilde{\pmb{X}}}_k$ as $\widehat{\tilde{\pmb{X}}}_k
	=
	\big(
	\widehat{\pmb{A}}_k^H
	\widehat{\pmb{A}}_k
	\big)^{-1}
	\widehat{\pmb{A}}_k^H
	\pmb{Y}_k$. 
	Next, one can fit the obtained $\widehat{\tilde{\pmb{X}}}_k$ via the model it follows in equation \eqref{eq:xlmk1-offset2} herein, as follows
	\begin{equation}
	\label{eq:joint-offset-delay-doppler-estimation2}
	\hat{\pmb{d}}^{\tt{tar}},
		\hat{\pmb{d}}^{\tt{u}},
		\hat{\pmb{d}},
		\hat{\pmb{f}}_D,
		\hat{\pmb{\sigma}}_{\tt{RCS}},
		\hat{\pmb{\delta}}^\tau,
		\hat{\pmb{\delta}}^f
		=
		\argmin_{		\pmb{d}^{\tt{tar}},
		\pmb{d}^{\tt{u}},
		\pmb{d},
		\pmb{f}_D,
		\pmb{\sigma}_{\tt{RCS}},
		\pmb{\delta}^\tau,
		\pmb{\delta}^f}
		\sum_{k=0}^K 
		 \Bigg\Vert
		\widehat{\tilde{\pmb{X}}}_k
		-
		\tilde{\pmb{X}}_k
		\Big(
		\pmb{d}^{\tt{tar}},
		\pmb{d}^{\tt{u}},
		\pmb{d},
		\pmb{f}_D,
		\pmb{\sigma}_{\tt{RCS}},
		{\delta}^\tau_k,
		{\delta}^f_k
		\Big)
		 \Bigg\Vert^2,
	\end{equation}
	where in the above we have made explicit that $\tilde{\pmb{X}}_k$ in equation \eqref{eq:Xk-with-offsets2} herein depends on the distances (equivalently delays and gains), dopplers, RCS values, as well as time and frequency offsets. 
	 $\pmb{d}^{\tt{tar}}$ is a vector containing all target distances, i.e. ${\tau}^{\tt{tar}}_1 \ldots {\tau}^{\tt{tar}}_q$.
	The vector $\pmb{d}^{\tt{u}}$ is a vector containing all user distances, namely ${\tau}^{\tt{u}}_1 \ldots {\tau}^{\tt{u}}_K$. 
	The vector $\pmb{d}$ is a vector containing all user target-user distances. As a reminder, we have that $\phi_{k,i} = \frac{d_{k,i} + d_i^{\tt{tar}}}{c} = \tau_{k,i}+\tau^{\tt{tar}}_i$.
	The vector $\pmb{f}_D$ contains dopplers of all the targets.
	The vector $\pmb{\sigma}_{\tt{RCS}}$ contains all  target \ac{RCS} values. 
	The vectors $\pmb{\delta}^\tau,
		\pmb{\delta}^f$ contain all the $K$ time offsets and $K$ frequency offsets, respectively.
	The optimization problem in \eqref{eq:joint-offset-delay-doppler-estimation2} herein is too complex to solve. Instead, we note that $\tilde{\pmb{x}}_{\ell,m}^{(k)}$ can be written in terms of its synchronized version as 
 \begin{equation}
 	\tilde{\pmb{x}}_{\ell,m}^{(k)}
 	=
 	{\pmb{x}}_{\ell,m}^{(k)}
 	 \exp(-j 2 \pi m \Delta_f \delta_\tau )
 	 \exp(j 2 \pi \ell T \delta_f)
 	 =
 	 {\pmb{x}}_{\ell,m}^{(k)}
 	 \exp(j 2\pi (-m \Delta_f \delta^\tau_k + \ell T \delta^f_k) ),
 \end{equation}
 where ${\pmb{x}}_{\ell,m}^{(k)}$ is obtained by setting $\delta^f_k$ and $\delta^\tau_k$ to zero in equation the expression of $\tilde{\pmb{x}}_{\ell,m}^{(k)}$ herein. 
 Using this, we can decouple the search per user while searching for $\delta^f_k$ and $\delta^\tau_k$.
 We experiment the estimator in \eqref{eq:joint-offset-delay-doppler-estimation2} for $K = 1$ user and $q = 1$ target, where the user is placed at $\hat{d}_1^{\tt{u}} = 100$m away from the \ac{DFRC} \ac{BS}. 
 We set $\delta^f_1$ to $5$ppm, which corresponds to $\delta^f_1 = 120$KHz at $24$ GHz. 
 We set $\delta^\tau_1 = 0.3\mu$sec.
 In Fig. \ref{fig:NMSE-FO}, Fig. \ref{fig:NMSE-TO}, and Fig. \ref{fig:NMSE-distance}, we plot the \ac{NMSE} for all three parameters, which are defined as follows
 \begin{equation*}
	\NMSE(\hat{\delta}^f_1)
	=
	\frac{1}{E}
	\sum_{e = 1}^E
	\frac{\Vert \delta^f_1 - \hat{\delta}^f_1(e) \Vert^2}{\Vert \delta^f_1 \Vert^2},
 \end{equation*}
  \begin{equation*}
	\NMSE(\hat{\delta}^\tau_1)
	=
	\frac{1}{E}
	\sum_{e = 1}^E
	\frac{\Vert \delta^\tau_1 - \hat{\delta}^\tau_1(e) \Vert^2}{\Vert \delta^\tau_1 \Vert^2},
 \end{equation*}
   \begin{equation*}
	\NMSE(\hat{d}_1^{\tt{u}})
	=
	\frac{1}{E}
	\sum_{e = 1}^E
	\frac{\Vert {d}_1^{\tt{u}} - \hat{d}_1^{\tt{u}}(e) \Vert^2}{\Vert {d}_1^{\tt{u}}\Vert^2},
 \end{equation*}
 where $\hat{\delta}^f_1(e), \hat{\delta}^\tau_1(e),$ and $\hat{d}_1^{\tt{u}}$ are the estimated values of ${\delta}^f_1(e), {\delta}^\tau_1(e),$ and ${d}_1^{\tt{u}}$ at the $e^{th}$ monte carlo simulation, respectively, through the multi-dimensional search adopted in \eqref{eq:joint-offset-delay-doppler-estimation2} herein.
 We can see that the method can give satisfying results for high \ac{SNR}, which has a positive effect on distance estimation as shown in Fig. \ref{fig:NMSE-distance}.
 In an ongoing paper, we intend to perform doppler and distance estimation by including the synchronization issue for the bistatic counterpart. We are currently preparing the paper that includes these topics.  
}

\textcolor{darkgreen}{We would have indeed liked to include this section, however since ToA and doppler is not our primary estimation focus in this paper, we will address synchronization issues in a follow-up paper.\\}

==> actions02/summary-of-actions.tex <==
In light of the reviewer's comment, we summarize our action items as follows:
\begin{itemize}
%	\item We have ran new simulations to study the gains from \ac{HRF} as a function of  \ac{BS} transmit power by fixing the powers of the users. We have used simulation parameters of a typical \ac{mmWave} system. We can see that at very high transmit \ac{BS} power, the \acp{CRB} will all converge to the same values, meaning that at very large \ac{BS} power, there will be no \ac{HRF} gains, signifying that it will not be necessary to fuse the received signals of the two links. However, if we focus on a typical \ac{mmWave} value of transmit power $40\dBm$, then we can still report some gains with increasing number of communication users.
 \item	If we focus on a typical \ac{mmWave} value of transmit power $40\dBm$, \ac{HRF} provides performance gains with increasing number of communication users. However, in the extreme case, at very high transmit \ac{DFRC} \ac{BS} power, the \acp{CRB} will all converge to the same values, meaning that at very large \ac{BS} power, there will be no \ac{HRF} gains, signifying that it will not be necessary to fuse the received signals of the two links. This has been validated through new simulations.

	\item We have added some discussion regarding reflections being weaker than direct transmissions, which will influence other detection links. A promising direction that we learned, and we are currently working on as part of future work, is to integrate \ac{ADC} quantization effects (such as 1-bit or few-bit) \ac{ADC} by mapping the analog part in equation \eqref{eq:rx-OFDM-UL} to equation \eqref{eq:sample-rx-OFDM} of the manuscript through a quantization function $\mathcal{Q}(.)$ (e.g. uniform mid-rise quantizer \cite{8171203} or the extreme 1-bit \ac{ADC} case, i.e. a simple comparator \cite{mezghani2018blind}) that would allow us to analyze the estimation limits as a function of ratios of user-BS to user-target-BS powers, in practical systems (i.e. \ac{HRF} with quantized outputs).
	\item We have ran new simulations to study when to abandon the smaller paths and focus on the larger paths, where simulation parameters of a typical \ac{mmWave} system have been used.  Indeed, when the paths are very weak compared to the \ac{LoS}, we can see that increasing the number of communication users will not yield significant \ac{MSE} improvement of the \ac{HRF} system. However, as the weaker paths become stronger, we can start observing the \ac{HRF} gain with increasing number of users. 
	\item We have showed the differences and advantages of different related works such as \cite{9805471} and \cite{9898900}.
	\item We have included how directional beamforming in Section VI can be adapted for beamscanning applications.
	\item We have corrected different mathematical typos and other typos as well.
%	\item We have summarized other parts, as well as introduced new acronyms to abide by the page limits (summarized parts are not in blue). 
\end{itemize}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> sections/introduction.tex <==
\IEEEPARstart{D}{\lowercase{espite}} having numerous similarities in terms of signal processing and system design, radar sensing and wireless communication have been evolving individually for many years \cite{9585321}. Interestingly, both radar and communication systems have quite a number of signal processing features that can be shared in common, thus favoring their joint design \cite{8999605,8828030,9705498,10041914,7786130,yu20226g,demirhan2022integrated}. Indeed, \ac{ISAC} can open the way for ground-breaking applications, for e.g., in the automotive sector \cite{9830717}, \ac{IoT}, and robotics.

%\ac{ISAC} collaboration and convergence is a pertinent feature that will open the way for ground-breaking applications, for example \ac{V2X} \cite{9606831}, due to its ability of performing high-rate communications and high-precision localization.

\ac{ISAC} has been investigated for different scenarios and challenges, including
\ac{NOMA} \cite{9668964,10024901}, 
holographic communications \cite{9724245}, 
optical fiber \cite{he2023integrated}, 
\ac{DFRC} \cite{9737357},
waveform design \cite{9724187},
\ac{UAV} \cite{10004900},
beamforming design \cite{10018908},
\ac{IoT} \cite{9206051}	, just to name a few. Due to the interoperability between the radar and communication sub-systems, \ac{ISAC} has a variety of tangible benefits, such as spectrum efficiency \cite{zhang2021overview}, less expensive modem by unifying hardware and software resources across \ac{SnC} tasks \cite{9830717}. These advantages bring a significant number of difficulties and research issues that must be resolved, such as the trade-offs between high data rates and high-resolution sensing. One of the earliest appearances of \ac{ISAC} was in the 60s \cite{4337601}, where \ac{SnC} tasks share the same power, spectrum and resources. In particular, pulse interval modulation was used for radar pulses and communication was embedded in those pulses. Owing to advances in waveform design, beamforming, and \ac{SDRs}, \ac{ISAC} has become a reality.

\ac{ISAC} can be categorized into three main categories, from a design perspective. A \textit{joint design} approach aims at developing new waveforms intended for \ac{SnC}, while offering tradeoffs between different \ac{KPIs}, such as data rates, capacity, energy for communications and probability of detection and \ac{CRB} for radar sensing. For e.g., the work in \cite{bazzi2022integrated} proposes a joint design of \ac{SnC} waveforms with adjustable \ac{PAPR}, allowing trade-offs between radar performance, communication rate and \ac{PAPR}. Moreover, another design is \textit{radar-centric} \ac{ISAC}, where a radar waveform is considered and communication information is inserted onto the radar waveform \cite{7347464,7746568,9093221,10018010,7746569}. Finally, \textit{communication-centric} \ac{ISAC} takes a communication waveform, for example, \ac{OFDM} or \ac{OTFS}, and estimates sensing parameters based on channel information probed in that waveform. Here sensing is an "add-on". The interested reader is referred to \cite{bazzi2022ris,9109735} for communication-centric \ac{ISAC}. 

\ac{DFRC} is a design technique that integrates radar and communication functions using a common transmit/receive aperture \cite{8828023}. For radar, there are two common settings for radar: mono-static \cite{8944152}, where transmit and receive units are co-located and bi-static \cite{5089551}, where the units are separated. Moreover, active and passive transmissions \cite{8950300} are common in radar, with active radar \cite{6034675} exploiting a known waveform to estimate target sensing parameters. Passive radar \cite{6617097} uses remote transmitters to take advantage of properties on different bands without knowledge of a specific waveform. In this paper, herein, we propose a new scheme named hybrid radar that considers both mono-static and bi-static settings, where the \ac{DFRC} \ac{BS} acts as a mono-static radar and the users act as distributed bi-static radars in the \ac{UL} following a \ac{FDD} protocol.



%\ac{DFRC}, a design technique for integrating \ac{ISAC} tasks, simultaneously performs radar and communication functions using a common transmit/receive aperture \cite{8828023}. For the radar counterpart, two common settings are mono-static \cite{8944152} radar and bi-static \cite{5089551} radar. In the former, the transmitting and receiving radar units are co-located so that the distance between the two units is negligible, relative to their distance toward the target. In the latter, both units are separated by a significant distance. Even more, two types of transmissions are common in radar, namely active and passive. In active radar \cite{6034675}, the radar exploits a known transmitted waveform in order to estimate the sensing parameters of the targets through the echo return signal. On the other hand, passive radar \cite{6617097} allows the usage of remote transmitters, also called donors, in conjunction with active radars to make use of properties on different bands, without the knowledge of a particular waveform. Also, active/passive radar system \cite{8950300} is also possible, where the target is seen as a passive illuminator and the active radar transmitter is operating on the co-channel within the same frequency band. In this paper, herein, we propose a new scheme named hybrid radar that considers both mono-static and bi-static settings, where the \ac{DFRC} \ac{BS} acts as a mono-static radar and the users act as distributed bi-static radars in the \ac{UL} following a \ac{FDD} protocol.




\subsection{Literature Review}
\label{subsec:literature-review}
To unbolt the potential of sensing capabilities in \ac{ISAC} systems, various lines of research work have been conducted in the literature. In particular, the paper in \cite{9468975} exploits \ac{OFDM} based waveforms in the \ac{DL} only, from a mono-static radar perspective, and performs delay and \textcolor{blue}{Doppler} estimation via periodogram criterion, which is only optimal for a single target. In addition, the paper in \cite{9860521} considers a bi-static setting, in which \ac{SnC} tasks are performed in orthogonal sets of sub-carriers, where the sub-carriers allocated to sensing are distributed among antennas in an interleaved fashion. Besides, the paper in \cite{9937163} proposes an \ac{ISAC} multi-user \ac{IRS}-aided scheme, capable of carrying out \ac{UL} data communications, while simultaneously performing target localization. Moreover, \ac{OTFS} \cite{7925924,bomfin2021channel} for \ac{ISAC} systems have been proposed in \cite{9557830}, where \ac{UL}, as well as \ac{DL}, communications are considered for vehicular communication systems. Their work has led to a novel model for delay-Doppler domain characterization for channel estimation. In the \ac{UL} phase, the \ac{RSU} infers the delay-Doppler components associated with each path to form a map of the vehicular network. As for the \ac{DL}, the \ac{RSU} constructs beamformers based on the predicted sensing parameters. It should be noted that the joint exploitation of \ac{UL}/\ac{DL} data was not part of the framework. Nevertheless, \cite{9724260} investigates multi-beam systems for \ac{ISAC} for 5G-\ac{NR} using \ac{OFDM} waveforms. The \ac{BS} in this study is a mono-static one, and joint range and \ac{AoA} estimation are modeled as sensing parameters, which further assists the beam-scanning procedure. However, the framework utilizes only the \ac{DL} information, and therefore the \ac{UL} information available from different users is neglected. Meanwhile, \cite{10018908,liu2018toward} consider the joint design of beamforming for \ac{SnC} purposes, which is well-suited for beam-scanning applications. These frameworks also rely on \ac{DL}-only communication information for sensing purposes. Furthermore, from a physical-layer security \ac{ISAC} perspective, the work in \cite{su2022sensing} provides sensing estimation based on the eavesdropper location to improve the secrecy rate of the system. In short, the framework utilizes \ac{DL}-only information for the radar echo. To the best of our knowledge, there does not exist any \ac{ISAC} scheme in the literature that functions on a hybrid monostatic and bistatic mode and fuses \ac{UL} and \ac{DL} information to efficiently estimate target sensing parameters.
\textcolor{blue}{\input{actions02/reference-R1.tex}}

\subsection{Contributions}
\label{subsec:contributions}
In this paper, we propose a \ac{HRF} system model, that combines both monostatic and bistatic modes, where the \ac{DFRC} \ac{BS} exploits the echos due to the \ac{DL} communication signals, in conjunction with \ac{UL} signals from a set of users associated with the \ac{DFRC} \ac{BS}. Each communication user transmits \ac{OFDM} waveforms on its own resource band, where the \ac{DFRC} \ac{BS} then fuses the information from different resources to estimate \ac{AoAs} of the targets in the scene.
\input{actions01/comm-assisted.tex}To this end, we summarize our contributions as follows
\begin{itemize}
	\item \textbf{Hybrid Radar Model.} We coin the term \textit{hybrid} because of the diverse and distributed radar functionality considered in this paper, i.e. the \ac{DL} echo is associated with a mono-static radar setting, as the \ac{DFRC}'s transmit and receive units are assumed to be colocated. Meanwhile, a (user,\ac{DFRC}) couple is seen as a bi-static radar, as the user is seen as a radar transmit unit in the \ac{UL}, transmitting via an \ac{FDD} protocol through \ac{OFDM} communication signals, and the \ac{DFRC} receive unit is the radar receiver. The \ac{DFRC}'s sophisticated task is to fuse the hybrid data at its disposal to estimate \textcolor{blue}{target locations}. \textit{To the best of our knowledge, the estimation model that arises due to the hybrid nature appears in the literature for the first time.}
	\item \textbf{Fused Maximum Likelihood Criterion.} We derive the \ac{ML} criterion of the hybrid radar model, and highlight our interpretations, such as its resemblance with the classical \ac{ML} criterion and the additional terms due to the participation of the communication users in the \ac{UL}.
	\item \textbf{Fused and Efficient Estimators.} In light of the hybrid and dual nature of the available data, we propose two computationally attractive estimators. The first one explicitly tackles the \ac{ML} criterion through an iterative optimization procedure that alternates between the target and user spaces. The second is an iterative subspace estimator: inspired by the \ac{MUSIC} principle, we formulate novel optimization problems, which lead to a new iterative estimator that carefully projects and fuses target and user location estimates.
	\item \textbf{Extensive simulation results.} Various performance metrics evaluating sensing performance via \ac{OFDM} communication waveforms are studied through simulations, demonstrating the effectiveness of utilizing fused data for the hybrid radar model. Numerical results show performance gains in terms of \ac{MSE} of the estimated \ac{AoAs} for the targets, especially when more communication users participate in the \ac{UL}. 
\end{itemize}
%Furthermore, we reveal some important insights, i.e.
%\begin{itemize}
%	\item insight1
%	\item insight2
%	\item insight3
%\end{itemize}
 


\subsection{Organization and Notations}
The following paper is organized as follows. Section \ref{sec:system-model} introduces the \ac{HRF} system model. Section \ref{sec:fused-maximum-likelihood} derives the \ac{ML} criterion of the problem from a sensing perspective. Section \ref{sec:estimation} designs an efficient fused \ac{ML} estimator for \ac{AoAs} of the different targets. Section \ref{sec:estimation-subspace} designs an optimization framework to derive a fused subspace algorithm that iterates between user and target \ac{AoAs}.
Section \ref{sec:directional-beams} presents two transmit beamforming techniques to realize directional beams for \ac{HRF}.
Section \ref{sec:discussion} discusses receive hybrid beamforming as a solution to the power discrepancies between \ac{LoS} and scattered components.
 Our simulation findings are illustrated and analyzed in Section \ref{sec:simulations}. Section \ref{sec:conclusions} concludes the paper.



\textbf{Notation}: Upper-case and lower-case boldface letters denote matrices and vectors, respectively. $(.)^T$, $(.)^*$ and $(.)^H$ represent the transpose, the conjugate and the transpose-conjugate operators. The empty set is $\emptyset$. The cardinality of $\mathcal{C}$ is $\vert \mathcal{C} \vert $. The set of all complex-valued $N \times M$ matrices is $\mathbb{C}^{N \times M}$. The determinant is $\det()$. The trace is $\trace()$. The $N \times N $ identity matrix is $\pmb{I}_N$. The projector operator onto the space spanned by columns of $\pmb{A} \in \mathbb{C}^{N \times M}$ is $\pmb{P}_{\pmb{A}}$ and the corresponding orthogonal projector is $\pmb{P}_{\pmb{A}}^{\perp} \triangleq \pmb{I}_N - \pmb{P}_{\pmb{A}}$. We index the $(i,j)^{th}$ element of $\pmb{A}$ as $\pmb{A}(i,j)$. The $k^{th}$ column of $\pmb{A}$ is indexed as $\pmb{A}(:,k)$. The $\Span$ of $\pmb{A}$, denoted $\Span(\pmb{A})$ returns the column space of $\pmb{A}$. The Moore-Penrose pseudo-inverse of $\pmb{A}$ is $\pmb{A}^+$.

